A Bi-Step Grounding Paradigm for Large Language Models in Recommendation Systems

As the focus on Large Language Models (LLMs) in the field of recommendation intensifies, the optimization of LLMs for recommendation purposes (referred to as LLM4Rec) assumes a crucial role in augmenting their effectiveness in providing recommendations. However, existing approaches for LLM4Rec often assess performance using restricted sets of candidates, which may not accurately reflect the models' overall ranking capabilities. In this paper, our objective is to investigate the comprehensive ranking capacity of LLMs and propose a two-step grounding framework known as BIGRec (Bi-step Grounding Paradigm for Recommendation). It initially grounds LLMs to the recommendation space by fine-tuning them to generate meaningful tokens for items and subsequently identifies appropriate actual items that correspond to the generated tokens. By conducting extensive experiments on two datasets, we substantiate the superior performance, capacity for handling few-shot scenarios, and versatility across multiple domains exhibited by BIGRec. Furthermore, we observe that the marginal benefits derived from increasing the quantity of training samples are modest for BIGRec, implying that LLMs possess the limited capability to assimilate statistical information, such as popularity and collaborative filtering, due to their robust semantic priors. These findings also underline the efficacy of integrating diverse statistical information into the LLM4Rec framework, thereby pointing towards a potential avenue for future research. Our code and data are available at https://github.com/SAI990323/Grounding4Rec.

==> AAexperiment_backup.tex <==
% P5 full x
% Video Games full >
% Flan-T5 Full ... (10 days)
% SASRec --> pop
% tau > X
% LLaMA embedding --> SASRec
% 
% Movies Scaling Law  
% Video Games scaling law x
% encoder-decoder
% mapping space (not tokens)



\section{Experiments}
\label{section:exp}
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}


% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}
In this section, we conduct experiments to answer the following research questions: 
\begin{itemize}[leftmargin=*]

\item 
RQ1: How does the performance of our model compare to existing methods, when trained on a limited sample of 1024 data points, in two different testing scenarios: one where popular items dominate and another with a balanced distribution of items?



\item RQ2: 
How does the performance of our model trained with limited data compare to that of fully-trained traditional models in the same domain?
    
\item RQ3: 
How is the performance of our model while simultaneously grounding the LLM to different real-world item spaces?

\item RQ4:
Can the LLM-based recommendation model achieve significant performance improvement with increasing data similar to traditional models?


\item RQ5: To what extent does incorporating popularity information and collaborative features during model grounding improve its performance?




    % \item RQ1: On equivalent samples (1024) and a test set dominated by popularity, does our model has advantages over traditional models?
    % \item RQ2: On equivalent samples (1024) and a test set balanced across all items, does our model has advantages over traditional models?

    % \item RQ3: By introducing popularity information in a causal manner, whether it is able to further boost our model's performance on a dataset dominated by popularity?
    % \item RQ4: How is the performance of our model when conjunction training upon multi-domain data?
    % \item RQ5: Does utilizing our model relative to traditionally trained models with complete data yield divergences, and where do the disparities lie if any?
\end{itemize}



\input{FIgure_Table/pop_count}

\subsection{Experimental Settings}
\subsubsection{Datasets.} We conduct experiments on two datasets:
\begin{itemize}[leftmargin=*]
    \item \textbf{Movie.} This refers to the well-known benchmark dataset for movie recommendation --- MovieLens10M\footnote{https://grouplens.org/datasets/movielens/10m/}.
    
    \item \textbf{Games.} This is a video-games recommendation dataset from Amazon\footnote{https://jmcauley.ucsd.edu/data/amazon/} and we use its 5-core subset. 
\end{itemize}


We chose the two datasets intentionally, as they exhibit different characteristics with regard to popularity bias. 
The Movie dataset reveals a significant bias towards popular items, while the Games dataset demonstrates a lesser degree of bias. 
Figure~\ref{fig:pop_count} illustrates the frequency of interactions across items with different levels of popularity, confirming that the Games dataset presents a more equitable distribution of interactions between popular and unpopular items than the Movie dataset. 
This suggests a lower degree of popularity bias in the Games dataset. Additional statistics for both datasets are summarized in Table~\ref{tab:dataStatics}.

 





To simulate real-world sequential recommendation scenarios, we divided each dataset into 10 periods based on the timestamp of the interactions. Subsequently, we split the periods of each dataset into training, validation, and testing sets\footnote{Due to limitations in the inference speed of LLM models, we randomly sample 5,000 validation and testing interactions as the final validation and testing sets, respectively.} using a ratio of 8:1:1. This approach ensures that the predicted interactions during testing come after all interactions observed during training, preventing the leakage of the testing phase information~\cite{ji2023critical} during training model. This is more akin to real-world situations~\cite{refCTR,ji2023critical}.


% In order to better simulate sequential recommendation scenarios in the real world, for each dataset, we first sort the sequences according to their timestamps, and then divide them into train, validation, and test sets based on the ratio of 8:1:1, in accordance with their chronological order. 
% \zjz{This ensures that the predicted interactions during testing occur later in time than the interactions observed during training, which is more aligned with real-world scenarios.}
% Table.\ref{tab:dataStatics} shows the static information of two datasets.

\subsubsection{Evaluation Protocols.}
% 遵循先前的工作，我们通过在测试阶段向模型输入一个序列，然后让模型预测用户会交互的下一个物品是什么来度量模型的性能。
Following the previous work~\cite{DRO1, SASRec}, we take the input historical interaction sequence for each testing interaction as the set of interactions that happened immediately prior to it. This approach allows for the possibility of including interactions that occur during the testing phase in the input sequence. 
To evaluate the model's performance, we use two commonly used evaluation metrics: Hit Ratio (HR) and Normalized Discounted Cumulative Gain (NDCG), which we compute using the all-ranking protocol. In this protocol, all items that a user has not interacted with are considered potential candidates.
%Following previous work~\cite{SASRec}, we measure the performance of the recommendation model by inputting a sequence during the evaluation phase and letting the model predict the next item the user would interact with. 
% 为了高效地度量我们提出的方法在有流行度bias和无流行度bias下的性能，我们通过对验证集和测试集采样构造了有偏和无偏两种测试来度量我们模型的性能。
% \todo{To efficiently evaluate the performance of our proposed method under popularity bias and no popularity bias, we constructed biased and unbiased settings by sampling from the validation and test sets.}




% \begin{itemize}
%     % 对于每个数据集，我们在划分好的验证集和测试集中随机采样了5000个用户历史交互和next item对来度量模型在有popularity bias下的性能表现。
%     \item \textbf{Normal Test.} For each dataset, due to limitations in the inference speed of LLM models, we randomly sampled 5000 user histories and the next item pairs from the pre-defined validation and test sets to assess the model's performance under the normal item distribution
%     % 对于验证集和测试集，我们为其中出现的每一个作为预测结果的item选取一条样本构成新的验证集和测试集
%     \item \textbf{Balanced Test.} For each dataset, we select one user history and the next item pair for each item appears as a prediction result in the pre-defined validation and test sets to testify to the model's performance in an entirely balanced scenario.
%     % For the validation set and test set, for each item that appears as a prediction result, we select one sample to constitute a new validation set and test set.
%     % \item \todo{add a figure/table to show the popularity of the above two dataset} 
% \end{itemize}

% 我们使用了两个被广泛使用的指标来度量模型的性能：hit ratio 和 normalized discounted cumulative gain
% We utilized two widely-used metrics to measure the performance of the model: Hit Ratio (HR) and Normalized Discounted Cumulative Gain (NDCG).


\subsubsection{Compared Method}
To demonstrate the superiority of our method in sequential recommendation, we compare it against the following conventional sequential recommendation methods and state-of-the-art large language model-based sequential recommendation methods:


% To showcase the superiority of our network structure in comparison to sequential temporal recommendation methods, we conducted a comparative analysis of three classical temporal recommendation algorithms.
\begin{itemize}[leftmargin=*]
    \item[-] \textbf{GRU4Rec~\cite{GRU4Rec}.} This is an RNN-based model that uses Gated Recurrent Units (GRU) to encode the user's past interactions with items and generate recommendations based on the learned patterns.
    
    \item[-] \textbf{Caser~\cite{Caser}.} It is a CNN-based model that represents the sequence of recent items as an image and uses convolutional filters in both horizontal and vertical directions to capture sequential patterns.
    In our implementation, we use one vertical filter and 16 horizontal filters with searching the height in \{2, 3, 4\}.
    
    
    % It is a CNN-based sequential recommender, which embeds a sequence of recent items into an “image” in the time and uses CNN in both horizontal and vertical ways to learn sequential patterns. We implement it with one vertical filter and 16 horizontal filters with heights searched in \{2, 3, 4\}.

    \item[-] \textbf{SASRec~\cite{SASRec}.} This is a self-attention-based model that uses a causal (left-to-right) attention mechanism to learn sequential patterns and predict the next item. 
    
    

    \item[-] \textbf{GPT4Rec-LLaMA~\cite{GPT4Rec}} is a modified version of the language model-based recommendation approach, GPT4Rec. The original method uses GPT-2 to generate hypothetical "search queries" based on a user's historical data, which are then searched using the BM25 search engine\footnote{We use the Rank-BM25 package at \url{https://github.com/dorianbrown/rank_bm25}.} to retrieve recommended items. To ensure a fair comparison, we have replaced the GPT-2 model with the LLaMA-7B model and performed model tuning using the LORA technique.    
    
    % This is utilizing a language model to generate a query and then conducting a search within the items using the BM25~\cite{BM25} search engine. We implement the BM25 with Rank-BM25 package~\footnote{\url{https://github.com/dorianbrown/rank_bm25}}. To ensure a fair comparison, we replaced the GPT2 model from the original paper with the LLaMA-7B model and performed lightweight finetuning using LoRA.
\end{itemize}

We primarily utilize decoder-only LLMs as the backbone LLM model in our \textbf{GoalRec} method, given their prominent roles in the LLMs field. Specifically, we have chosen LLaMA-7B as our default choice for this study. However, to investigate the impact of LLM model architecture, we also implement an alternative version called \textbf{GoalRec-T5}, which uses an encoder-decoder type of LLM model - Flan-T5-11B, currently the top-performing model in the T5 series~\cite{T5}. In addition to GPT4Rec, there are other existing LLM-based recommendation methods, such as TALLRec~\cite{bao2023tallrec}. However, since these methods are not applicable to our all-ranking setting, we do not compare them in our study.

    % \item[-] \textbf{Flan-T5~\cite{T5}.} A recommender system based on an encoder-decoder architecture LLM, Flan-T5-11B, which is currently the best-performing model in the T5 series, is chosen for comparison as we directly applied our method to this model.

% \subsubsection{Implementation Details}
% % 
% Our study utilizes Python 3.10 and PyTorch 2.0 to implement the proposed methods. 
% In order to maintain consistent sequence lengths, we employ padding on sequences with a historical interaction length below a predetermined threshold of 10, utilizing `<pad>' tokens. 
% % For historical interaction sequences with a length greater than 10, we have retained the last 10 interactions as the historical sequence.
% \zjz{For user interaction history data with a length greater than 10, we utilized a sliding window of length 10 to construct the sequence that meets the length requirement.
% The model needs to predict the user's next interaction item based on the provided sequence.}
% For all traditional sequential recommendation baselines, we use Adam~\cite{Adam} optimizer, the learning rate is tuned as $1e-3$ and the batch size is set as 1024. We tune the weight decay within the range of $[1e-2, 1e-3, 1e-4, 1e-5, 1e-6, 1e-7]$. We use the early stop with a patience of 20 epochs to select the best model. We use binary cross-entropy loss and uniform negative sampling to optimize the traditional recommendation baselines since this is an implicit feedback setting.
% \zjz{We use single layer GRU for GRU4Rec suggested by~\cite{GRU4Rec}, single attention head for SASRec since~\cite{SASRec} shows it performs best, one block for SASRec since~\cite{SASRec} shows it is not sensitive to the number of blocks. Finally, we set the embedding size of all the traditional sequential recommendation baselines to 64 and the dropout ratio is 0.1.}
% For LLM-based methods, we follow the alpaca setting~\cite{alpaca}, directly set the learning rate to $1e-4$, and use the AdamW~\cite{AdamW} optimizer. \zjz{For the hyperameters of BM25, we follow the tuning range of GPT4Rec~\cite{GPT4Rec}.} We report the average results for three random seeds.
\input{FIgure_Table/tab_dataset_static}


\input{FIgure_Table/tab1}

\subsubsection{Implementation Details}
% 
We implement all of our methods using PyTorch. To preprocess the data, we first pad user interaction history with lengths less than 11 to a fixed length of 11. Then, we use a sliding window of length 11 to extract sequences, where the last item in each sequence is used as the prediction target and the preceding items form the input sequence. For all conventional models, we optimize them using the binary cross-entropy loss and uniformly sample negative samples. We use the Adam~\cite{Adam} as the optimizer with a tuned learning rate of $1e-3$, a batch size of 1024, and tune the weight decay in the range of $[1e\text{-}2, 1e\text{-}3, 1e\text{-}4, 1e\text{-}5, 1e\text{-}6, 1e\text{-}7]$. Regarding the hyperparameters of the conventional model architectures, we set their embedding size to 64 and the dropout ratio to 0.1. As suggested by the original papers, we only use one GRU layer for GRU4Rec; for SASRec, we set the number of self-attention heads and blocks to 1. For LLM-based methods, we follow the Alpaca setting~\cite{alpaca}, directly set the learning rate to $1e-4$, and use the AdamW~\cite{AdamW} optimizer. For the hyperparameters of BM25, we follow the tuning range provided in GPT4Rec~\cite{GPT4Rec} paper. For all methods, we use the early stop strategy with the patience of 20 epochs to select the best model and report the average results for three random seeds.




\input{FIgure_Table/Scaling_law}

\subsection{Performance Comparison with Limited Training Data (RQ1)}
We first follow existing work~\cite{bao2023tallrec} to study the effectiveness of our method with limited training data (1024 training points).  We compare it with the baselines trained with equivalent training samples. The comparison results results are summarized in Table~~\ref{tab:pop_1024}, where we draw the following main observations:
\begin{itemize}[leftmargin=*]
    \item When training data is limited, the conventional sequential baselines (GRU4Rec, Caser, SASRec) exhibit significantly worse performance than GoalRec implemented with decoder-only LLM. These results are not surprising as these baselines rely on ID embeddings to build a recommender model, which is difficult to learn well with limited data. In contrast, GoalRec rapidly leverages the semantic knowledge of LLM obtained during the pre-training phase to achieve effective recommendations. These findings demonstrate the superiority of GoalRec over traditional recommendation models when dealing with limited training data. Furthermore, the improvement of GoalRec over these baselines in the top-ranked positions is much higher, indicating that GoalRec may tend to rank items of interest to users in higher positions. 

    \item While GPT4Rec-LLaMA is also LLM-based, it exhibits poor performance compared to GoalRec. We attribute this to the fact that BM25, which is used to ground the LLM outputs into real-world items, is not suitable for the task. BM25 is a retrieval tool designed for document-level text. However, for the two datasets used in our study, the queries in GPT4Rec (item titles)  are very short. As a result, BM25 is susceptible to the impact of low-frequency word noise, making it difficult to accurately retrieve relevant items.

    \item  
    Despite using a larger Flan-T5-11B model and having relevant domain knowledge about the two datasets, GoalRec-T5, the encoder-decoder version of GoalRec, unexpectedly underperforms conventional recommender models. This may be attributed to inherent limitations of the encoder-decoder architecture, such as its relatively poor ability for generative tasks, as well as the potential need for more data to effectively learn a good sequence representation through the encoder.

    \item  The improvement of GoalRec over conventional models is significantly higher for the Games dataset compared to the Movie dataset. This difference is possibly due to the varying properties of popularity bias between the two datasets. Conventional methods tend to capture popular bias, while GoalRec is less affected by popularity bias. Therefore, conventional methods may perform better on the Movie dataset, in which popular items play more dominant roles as evidenced by Figure~\ref{fig:pop_count}.
    
%     Another interesting finding is that our model's performance enhancement over traditional models on Video Games is far more significant compared to the enhancement on MovieLens10M.
% There may have been multiple contributing factors, a key consideration is that MovieLens10M  is a popularity-dominated dataset, so even with 1024 samples, traditional models can learn some popularity knowledge through the frequency of ID appearances.
    

    % We attribute this phenomenon to the innate disadvantage of the encoder-decoder architecture for generative recommendation tasks with fewer samples, on the one hand, the encoder inevitably loses some information when aggregating information for all tokens, and on the other hand, obtaining a good user representation through the encoder may require more data to learn from.
    
\end{itemize}

\input{FIgure_Table/tab2}


% % 首先为了验证我们的方法的有效性，我们首先在相同的样本上与传统方法对比
% To ascertain the effectiveness of our proposed method, we initially compare it with traditional methods on equivalent samples (1024).
% % 表1展示了baseline方法和我们的方法在常规数据集上的表现
% Table~\ref{tab:pop_1024}  exhibit the performance of the baseline and our method on the normal test sets.
% % 首先我们可以观察到，在有偏数据上基于ID的baseline差距不是很明显, 说明了这些传统的推荐模型在少数据量上没有本质的差别
% Firstly, we observe that on the normal test set, the performance disparity of the ID-based baselines is not very pronounced, demonstrating that these conventional recommendation models lack intrinsic distinction in low-source settings.
% % 对比我们基于Decoder大模型的方法，情理之中的是大模型利用其在预训练阶段学到的知识能够更快的通过语义进行推荐，相比于传统模型有着明显的优势，然而其在头部的明显提升仍然在我们的意料之外
% Compared with our methodology leveraging a decoder-based LLM, it is reasonable that the LLM, by virtue of the knowledge obtained during the pre-training phase, may recommend more rapidly through semantics, manifesting a dominant over traditional recommendation models; yet, its salient improvement on the top-rank remains beyond our anticipation (Improved more than 600\% and 1000\% at NDCG@1 on the movie and video games dataset, respectively.

% % 令我们惊讶的事情是, 同样的基于大模型的方法, Flan-T5-11B的模型却并没有展现出任何优势, 甚至比传统的推荐模型还要差, 尽管从参数量上他要大于LLaMA7B, 同时他也具有一定的领域知识(例如，询问Flan-T5-11B什么是钢铁侠，他能给出钢铁侠电影的相关知识）
% What did surprise us is that the identical methodology leveraging Flan-T5-11B, failed to learn to recommend in a low-resource setting, in fact performing worse than traditional recommendation models, despite it being larger in parameters compared to LLaMA-7B and also possessing some domain knowledge (for instance, upon asking Flan-T5-11B what is Iron Man (II), it can furnish relevant information about the Iron Man (II) movie).
% % 我们将这个现象归因于encoder-decoder架构对于生成式推荐任务在少样本上的天生劣势，一方面，encoder在对所有token做信息聚合的时候难免会丢失一部分信息，另一方面，通过encoder获得一个很好的用户表示可能需要更多的数据量来学习
% We attribute this phenomenon to the innate disadvantage of the encoder-decoder architecture for generative recommendation tasks with fewer samples, on the one hand, the encoder inevitably loses some information when aggregating information for all tokens, and on the other hand, obtaining a good user representation through the encoder may require more data to learn from.
% % 而另一个基于大模型的方法GPT4Rec-LLaMA, 同样表现出很差的推荐能力，我们认为这是因为BM25本身是一个适用于长文本检索的检索工具，而在电影和游戏领域，由于标题长度本身较短，因此BM25很容易受到低频词噪声的影响从而难以做到准确的召回
% While another LLM-based method GPT4Rec-LLaMA also exhibits poor recommending capability which we attribute to the fact that BM25 is a retrieval tool apt for document-level text.
% In domains like movie and video games, due to the inherent short length of titles, BM25 succumbs to the impact of low frequency word noise, making it difficult to accomplish accurate recall.
% % 另一个有趣的发现是，我们的模型在Video_Games上相比于传统模型的性能提升要远高于在MovieLens10M上相比于传统模型的提升
% Another interesting finding is that our model's performance enhancement over traditional models on Video Games is far more significant compared to the enhancement on MovieLens10M.
% % 这个原因可能归结于多方面，一个重要的考量是流行度是否主导了该数据集的推荐结果. 
% There may have been multiple contributing factors, a key consideration is that MovieLens10M  is a popularity-dominated dataset, so even with 1024 samples, traditional models can learn some popularity knowledge through the frequency of ID appearances.

% 为了进一步观察这个现象，我们在表2中展示了baseline模型和我们的模型在一个对于item来说均衡的数据集上的表现
\par \textit{Performance on Balanced Testing.} 
To further validate that our method is less susceptible to the popularity bias of the training dataset, we performed an additional experiment using a balanced testing setting. We followed the approach described in MACR~\cite{MACR} to adjust the testing distribution of items to be uniform and evaluated the model's performance. A model that is less affected by the popularity bias in the training data is expected to perform better in this balanced setting. We have summarized the results of all compared methods in Table~\ref{tab:unpop_1024}.

As shown in the table, all models experience a noticeable decrease in performance compared to their results on the normal test setting presented in Table~\ref{tab:pop_1024}. This can be attributed to the models' lack of knowledge about tail items or their inability to utilize the knowledge stored in LLMs for recommendation. However, in this balanced testing setting, the performance improvement of GoalRec over conventional baselines is even greater than that observed in the normal test setting in Table~\ref{tab:pop_1024}. This suggests that GoalRec may be superior for tail items, indicating that it is inherently less sensitive to the popularity bias of training data when compared to conventional recommendation models.




% To further observe this phenomenon, we demonstrate the performance of the baseline model and our methods on a balanced test set for items in Table~\ref{tab:unpop_1024}. This because 



% However, 
% % 尽管我们观察到所有的模型相比于Normal的test set都有明显的下降, 这是由于在1024样本上很多样本是模型没有见过的，因此无论是大模型还是小模型都不知道可以把这类样本放进结果空间中考量
% Although all models exhibited a noticeable drop compared with their performance on the normal test set, mainly because both the baseline models and LLMs are not seen many items before; therefore, they are not likely to know how to consider such items in their result spaces. However, 
% % 尤其是对大模型来说，即使他有这个item的信息，他仍然不知道怎么怎么把这个item考虑成一个结果
% Notably for the LLMs, even when they had the requisite item knowledge, they still did not know how to consider that item as a solution for the recommendation problem at hand.
% % 然鹅，我们仍然发现了大模型相比于传统模型的巨大提升，甚至比他在normal测试集上的提升还要明显
% However, we are still nevertheless delighted to discover that the LLM shows a greater improvement over these traditional models, even higher than that improvement on the normal test set, over 4000\% improvement for both scenarios.
% % 这表明了相比于传统模型，大模型在学习过程中确实不易收到pop的影响
% This indicates that the LLMs are innately less sensitive to popularity information in the learning process when compared to the traditional recommendation models.



% \subsection{Popularity Effectiveness for GoalRec (RQ2)}
\subsection{Performance of Popularity Augmented Grounding (RQ2)}
% 前文分析到了大模型的推荐结果天然对于流行度不敏感，但是在某些场景下面流行度有比较重要比如流行度主导的movie数据集。那么是否有可能将流行度信息引入到大模型推荐中去呢？我们发现直接在grounding to the reality阶段通过简单使用类似于PDA~\cite{PDA} 的方式，就可以使得大模型能够利用流行度提高推荐性能。

The preceding analyses highlight the insusceptibility of GoalRec to popularity bias during learning. However, in certain scenarios, such as when higher popularity represents current trends and better intrinsic quality, incorporating some popularity bias can be helpful in improving recommendation accuracy, as discussed by PDA~\cite{PDA}. To further investigate this, we studied whether using the method presented in Equation~\ref{eq:eq2} to incorporate popularity information into the grounding of GoalRec could enhance its recommendation accuracy for Movie data, where popular items are particularly important. We compared the original version of GoalRec with the version that incorporates popularity information in Figure~\ref{fig:pop_enhanced}. 
The figure demonstrates that after incorporating popularity information, GoalRec achieves performance improvements for the NDCG@K and Recall@K metrics, particularly for larger values of $K$. Additionally, the performance is substantially better than when using only popularity information for recommendation (as shown in Table~\ref{tab:full_training_result}). These results indicate that injecting popularity information can be beneficial for grounding the output of LLMs to real-world items in GoalRec, further enhancing its performance.



 Additionally, the utilization of the simple approach outlined in Equation~\ref{eq:eq2} for adjusting the grounding of GoalRec has resulted in improved performance. This indicates that there is significant potential for advancing recommendation accuracy even further by investigating more effective and efficient techniques for enhancing the grounding to the real-world item space in GoalRec.


\input{FIgure_Table/RQ3_figure}




% The previous analysis highlighted the insensitivity of GoalRec towards popularity bias, but in certain scenarios, such as popularity-driven movie datasets, popularity can be quite important. 
% Is it possible to incorporate popularity information into the recommendations generated by LLMs? Our analysis in the grounding to the real-world stage indicates that simply utilizing a method similar to PDA~\cite{PDA} can enable large models to leverage popularity to enhance the performance of recommendations~\footnote{\zjz{
% We performed tuning $\gamma$ for each K based on the validation set performance using the parameter range specified in PDA~\cite{PDA}.}}. 
% % 考虑到这个实验分析的是在流行度重要的情景中的结果，我们在流行度主导的movie数据集上进行了测试。
% Given that this experiment examines the outcomes in a context where popularity is paramount, we conducted our testing on the movie dataset which is dominated by popularity.
% % 因为我们探究的是融入流行度增强模型性能的可行性，我们对每个K按照PDA~\cite{PDA}中的调参范围进行了调节。我们的实验证明了可以在grounding to the real-world阶段加入传统推荐中重要的统计信息比如流行度来增强模型的推荐性能，为未来进一步的探索提供了想象空间。

% % \todo{Detail setting for pop GoalRec}

% Based on the result, we have the following observations:
% \begin{itemize}
%     % 加入流行度之后，在K比较大的时候有明显的提升。这也符合之前的分析，大模型自然擅长K很小的推荐，加入流行度后有助于提高top 20这种相对比较大的K的推荐性能。
%     \item After incorporating popularity, there was a noticeable increase in performance when K was relatively large. This aligns with our previous analysis that LLMs are naturally better at recommending for smaller values of K, and adding popularity helps to improve the recommendation performance for larger values of K such as the top 20.
%     % 加入流行度之后，尾部的性能同时比直接使用GoalRec进行推荐和使用流行度推荐都高，这说明grounding to the real world 阶段的模型可以从流行度中受益，同时结合GoalRec和流行度的有点。
%     \item After incorporating popularity, the performance of the model on the tail end is higher compared to using either GoalRec or popularity-based recommendations alone. This indicates that the grounding to the real-world stage of the model can benefit from popularity, as well as the combination of GoalRec and popularity.
% \end{itemize}
\input{FIgure_Table/RQ4_figure}


\input{FIgure_Table/tab3}


% \subsection{Is Multi-Domain Decrease the Performance?(RQ4)}
\subsection{Performance of Grounding to Multiple Real-World Item Space (RQ3)}
% LLMs 除了能够快速学会一个新的任务以外，还具有极强的跨域泛化能力。为了验证在经过我们提出的grounding范式之后，LLM是否还保留类似的能力，我们构建了一个multi domain的测试场景。
% LLMs have a good property in addition to being able to quickly learn a new task, which is that they could serve as a universal processor for different tasks. It is doubtful whether LLMs still retain similar capabilities after applying our grounding paradigm, \ie whether we can simultaneously ground LLMs to different recommendation spaces. To study this, we randomly select 1024 samples from the two-domain datasets (Movies and Games) to train our model and then test the trained model on each testing set, comparing the performance with the model trained with the single-domain data. The results are illustrated in Figure.\ref{fig:multi_domain_result}.  We find that GoalRec trained on two-domain data can achieve comparable performance on each individual domain as compared to when it is trained on a single domain. These results verify that GRec can simultaneously ground LLMs to different recommendation spaces, at least, different domain recommendation spaces.
 In addition to their ability to quickly learn new tasks, LLMs have the potential to serve as a universal processor for different real-world item spaces.
 However, it is unclear whether this capability is retained after applying our grounding paradigm, \ie whether our grounding paradigm can ground LLMs to different real-world item spaces simultaneously. 
 To explore this, we randomly selected 1024 samples from two domains (Movies and Games) to train our model and tested it on the testing sets of two domains, respectively.
 We compared the performance of this model with the model trained on single-domain data. 
 The results, depicted in Figure \ref{fig:multi_domain_result}, demonstrate that GoalRec trained on two-domain data performs comparably on each individual domain as compared to when it is trained on a single domain. 
 These findings suggest that GoalRec can simultaneously ground LLMs to different real-world item spaces, at least at the level of different domains.






% LLMs exhibit robust cross-domain generalization abilities in addition to being able to quickly learn new tasks. To determine whether LLMs retain similar capabilities after undergoing our proposed grounding paradigm, we devised a multi-domain testing environment.
% %具体而言，我们首先从movie和games两个数据集中随机选出1024个samples，合在一起构造数据供大模型进行instruction tunning训练，然后我们分别在movie和games单独测试训练好的模型，查看它相对于只在单个数据集上训练，单个数据集上测试的结果的变化。
% To be specific, we initially selected 1024 samples randomly from the movie and games datasets and combined them to form data for the LLM to undergo the instruction-tuning phase. 
% Subsequently, we test our models separately on the movie and games datasets to observe the changes in the results compared to those obtained from training and testing on a single dataset. The results are illustrated in Figure.\ref{fig:multi_domain_result}. 



% % 我们从实验结果中最主要的观察是我们提出的GoalRec在使用两个domain进行训练之后，可以分别在两个domain上取得和单个domian上训练推荐相当的性能，这体现了我们提出的GoalRec的强大的跨域推荐性能。
% The primary observation from our experimental results is that our proposed GoalRec model, after being trained on two domains, can achieve comparable performance on each individual domain as compared to when it is trained on a single domain. This highlights the robust cross-domain recommendation performance of GoalRec.
% % 具体而言，Figure中每个柱子的左边是multi domain训练，单个domain测试的结果，右边则是直接在该domain上训练并测试的结果。我们展示了两个数据集中不同K的NDCG和HR的结果。可以看见在所有情况下，GoalRec并没有因为domain变多而导致推荐性能出现显著下降而是体现出和comparable的结果
% To be precise, the left side of each bar in Figure.\ref{fig:multi_domain_result} shows the results of multi-domain training and single-domain testing, while the right side shows the results of training and testing directly on that domain. We present the NDCG and HR results for different values of K in two different datasets. 
% In all scenarios, it can be observed that GoalRec did not exhibit a significant decrease in recommendation performance due to the increase in domains, but rather demonstrated comparable results.





\subsection{Performance Comparison to Full-Data Training Baselines (RQ4)}
% 我看摘要里面这样提的，统一一下
% 基于大模型在相同数量sample上的表现如此炸裂，一个自然的想法是与更多训练数据量相比的传统模型比较，在少量样本上训练的大模型还有多少差距
Given the impressive performance gains of GoalRec over baselines when trained on limited data, we are curious to investigate the extent of the gap that remains between GoalRec trained on limited data and the baselines trained with full training data.
Table~\ref{tab:full_training_result} presents the results of the baselines trained with full data, which consisted of over 7 million sequences for Movies and 120 thousand for Games, alongside the results of GoalRec trained with only 1024 samples. 
From the table, we find that, compared to conventional baselines on the Movie data, GoalRec exhibits better performance at the top position of the recommendation list, but performs worse with regard to the relative bottom positions of the recommendation list. Contrasting with the findings for the movie dataset, on the Video Games data our method exhibits consistently superior performance to traditional models. We draw two conclusions based on these results:
\begin{itemize}[leftmargin=*]
    \item Our method, GoalRec, trained on just 1,024 samples, could demonstrate comparable performance to fully-trained conventional models in most cases, particularly when recommendation resources are limited. This highlights the practical applicability of LLMs for recommendations. Meanwhile, the results indicate that there is significant potential to enhance GoalRec's grounding by enlarging its training set and expanding its seen real-world items during grounding, which may lead to further performance improvements.
    
    \item When compared to the Games dataset, the Movie dataset is denser and more heavily influenced by popularity bias (as evidenced by the performance of the Most-Pop methods on the two datasets). The difference in the performance gain of GoalRec between the two datasets suggests that GoalRec performs exceptionally well in scenarios where data is scarce and works effectively with less reliance on popularity bias.
    
    % The superior performance of traditional models at the relatively top positions of recommendation lists in the MovieLens10M (@10 and @20), in addition to being attributable to data density and volume factors, may also stem from the effect of popularity on this particular data set. As shown in the table~\ref{tab:full_training_result}, a naive recommendation method based solely on popularity (Most-Pop) proves notably effective for MovieLens10M.
\end{itemize}


% Given the explosive performance of the LLMs on the equivalent number of samples, a natural idea is to compare them to traditional models trained with far more data to gauge how much of a gap still remains for large models trained on small amounts of data.
% % 表3展示了大模型在1024个样本上训练的结果对比传统模型在所有sequence上训练的结果(8M for MovieLens10M, 110K for Video Games) PS: 这里只有训练集，没有用验证集和测试，比所有seq总数少
% Table 3 illustrates the performance of the LLMs, which are fitted employing a mere 1,024 samples, in apposition with the outcomes attained by traditional models that are trained on the entirety of the available sequences (amounting to over 7 million sequences for MovieLens10M and 120 thousand for Video Games)

% % 在电影数据集上，我们发现与传统模型相比，基于LLM的模型在头部仍然有巨大的性能提升，这表明了利用大模型的生成能力进行推荐的可行性
% On the movie dataset, we find that, in comparison to the traditional models, the LLM-based models fitted by our methodology continue to exhibit superior performance in the top ranks (over 200\% improvement on NDCG@1), indicating the feasibility of harnessing the generative capabilities of LLMs for recommendations.
% % 除此以外，我们发现传统模型相比于大模型的优势在于相对靠后的排序位置，这表明了基于大模型的生成式推荐仍然有很大潜力可以挖掘。
% In addition, we find that traditional models exhibited an advantage over LLMs with regard to the relative position of lower-ranked recommendations, indicating that there remains great untapped potential in generative recommendations based on LLMs.
% % 与电影数据集不同，在Video Games数据集上，我们的模型与传统模型在各个rank上有着一致的提升
% Contrasting with the findings for the movie dataset, on the Video Games data our methods exhibit uniformly superior performance to traditional models.

% 综合上面两个数据集来看，我们有以下总结
% Upon reviewing the findings across the two datasets, the following conclusions may be drawn:
% % 从整体上来看，我们的模型在1024样本上训练后的表现与传统模型在两个数据集上全量数据训练后的的表现相近，
% \begin{itemize}
%     \item 1) Our methods with training on a mere 1,024 samples show comparable performance \zjz{in most cases} with that of traditional models trained on the entirety of the two datasets, demonstrating the practical applicability of LLMs for recommendations, suggesting 
% % 在电影数据集上传统模型在相对考后的排序位置的表现, 除了数据抽密度和数据量的关系以外，还有可能源自于流行度对这个数据集的影响，如表中所示仅仅通过流行度的推荐方法(Most-Pop)明显更实用与MovienLens10M
%     \item 2)The superior performance of traditional models at the relative position of lower ranks in the MovieLens10M (@10 and @20), in addition to being attributable to data density and volume factors, may also stem from the effect of popularity on this particular data set. As shown in the table~\ref{tab:full_training_result}, a naive recommendation method based solely on popularity (Most-Pop) proves notably effective for MovieLens10M.
% \end{itemize}
% \todo{Ground vs Alignment
% Gournd abstract --> Concrete
% Alignment abstract --> abstract}


==> AAinto-backup-0714.tex <==

% 尽管大模型本身可能缺乏对推荐任务的认知，但是研究者们指出仅仅需要通过少量样本就能让大模型学会推荐，这种能力能够 (
% Albeit the LLM may lack cognizance of recommendation tasks, scholars note that merely requiring a meager number of samples suffices to let the LLMs learn the recommendation, which will be able to usher recommendations into an entirely novel age~\cite{}.

\section{Introduction}
% 现在大模型在各个领域展现出其强大的能力 (大背景)
Nowadays, Large Language Models (LLMs) exhibit their mighty powers across multiple domains. 
% 在实验中人们发现了大模型展现了强大的上下文理解能力和语言生成能力，人们可以仅仅通过自然语言的指示来要求大模型完成各种各样的任务 (指出ICL和Instruction-tuning)
In practice, LLMs demonstrate enormous contextual comprehension and generation capabilities, allowing individuals are able to command the LLMs to carry out diverse tasks well via straightforward natural language instructions~\cite{}.
% 更近进一步来说，研究者们指出，LLM拥有基于真实世界的知识进行推理的能力以及仅仅通过少量样本学会一个新任务的能力 (指出我们依赖的两个能力)
Furthermore, different from traditional language models (e.g. BERT~\cite{}, GPT2~\cite{}), researchers have pointed out that LLM possesses the ability to reason based on real-world knowledge and the ability to learn a new task with just a small amount of samples.
% 目前，在推荐领域，研究如何更好的利用大模型进行推荐正在蓬勃发展 (引入推荐）
Currently, in the field of recommendation, studies exploring utilizing LLMs for better recommendations are also developing vigorously~\cite{}.

% 在这么一个重要的领域，一个很有价值的问题是，LLM究竟给推荐领域带来了什么样的可能性，以及我们如何在推荐任务中好好利用LLM (引出问题）
Within this important research direction of LLMs for recommendations (LLM4Rec), a valuable issue is, 
what novel possibilities have LLMs brought to the domain of recommendation and how can we make use of LLMs greatly in the recommendations? 





% 第二段  说现有的研究工作
%在最近的研究工作中， 有大量的工作尝试将LLM引入推荐领域, 这些工作主要分为两个流派
In recent attempts, there have been a lot of works aimed at introducing LLMs into recommendations, which principally break into two groups -- In-context Learning based and Instruction-tuning based~\cite{}.
% - in-context learning 通过调用API和给予LLM case来完成推荐
For the former, they attempt to call an accessible API (e.g. ChatGPT), and by giving the model several recommendation examples request the LLM to conduct recommendatoins~\cite{}.
% 这一类的问题是，推荐任务和LLM的预训练任务差别较大，很难通过简单的prompt去消除gap， leading to inferior performance. 
% 这一类方法的问题是，由于LLM的预训练任务与推荐任务gap较大，缺乏特定推荐领域的知识， 我们很难通过简单的prompt来消除这种gap，leading to an inferior performance.
% Yet owing to the lack of specific domain recommendations such methods hardly achieve noteworthy results.
Yet owing to the fact that there exists a gap between the pre-training task of LLms and the recommendations, the LLM lacks domain-specific recommendation knowledge, which is hard to eliminate this gap through a simple prompt, eventually resulting in an inferior performance.
% - Instruction-tuning based methods.  人们通过instruction tuning教会LLM 推荐任务
For the latter, researchers try to teach the LLM how to recommend through instruction tuning and get a promising result~\cite{bao2023tallrec}.
%  然而上述两个方向，模型都仅仅表现出有限的性能
However, current models only show a limited recommendation performance.
Additionally, current researchers often delimit the range of items visible to the model which is difficult to show the real performance of the recommendation ability of LLMs.
% by using point-wise, pair-wise or list-wise recommendations 
% 他们中的一部分人尝试利用推荐数据，通过instruction-tuning微调大模型来使得大模型学会推荐任务
% 尽管大量先前的工作已经初步验证了，利用将大语言模型应用到推荐领域能在
% 但是他们往往忽视了LLM是一个生成模型，而选择让LLM做选择和排序（抑制能力），因此通过这种方式分析LLM应用到推荐的可能性可能并不靠谱






%由于现有的基于LLM的方法在推荐任务上仅仅展现了limited performance，我们迫切的想要利用好大模型进行推荐, 换句话说我们希望将LLM ground to Rec, which means we need to find a way to transfer the output of the LLM to a meaningful items in the real-world.
% Due to the existing LLM-based methods displaying limited performance in recommendation tasks, we ardently desire to leverage LLMs to enable effectual recommendations.
% 我们将他们不高的表现归因于，预训练阶段和指令微调阶段的不一致性
In general, we attribute this inferior performance to their disagreement between the pre-training phase and the instruction-tuning phase.
% 换句话说  我们应当使用与预训练保持一致的生成模式来进行推荐来弥补这个gap
Therefore, we should be in consonance with the training mode of the pre-training stage and employ a generative modality that directly yields the next item to minimize this gap to assist us in better utilizing LLM to the recommendation.
In other words, we ought to ground the LLM to the recommendation, by transferring the output of the LLM to a meaningful item in the real world for recommendation. 
% 一个显而易见的想法是，为了尽可能运用大模型在预训练阶段得到的能力，我们应当尽量减少预训练任务和推荐任务之间存在的gap来帮助我们更好的LLM ground到推荐上来，因此遵循预训练阶段的训练要求，我们使用一个generative 的 manner直接生成下一个item是自然的选择
% An evident notion is that, for the sake of utilizing the abilities obtained from the pre-training phase as much as possible, we should minimize the gap existing between the pre-training phase and the recommendation tuning phase to assist us in better grounding the LLM to the recommendation.
% Therefore, in consonance with the training mode of the pre-training stage, employing a generative modality that directly yields the next item is an instinctual option.
% 但是呢，直接通过生成的方式将生成结果限制到具体的item上是很难的一件事，除此以外，如果限制死了模型的生成范围，一个新来的item即使模型认识也很难对其进行适配
However, owing to the creative generative capabilities of the LLM, directly restricting the generated outputs to a specific item set is a difficult task; moreover, overly restricting the model outputs means that it will struggle to adapt to a novel item, even though the LLM recognizes it.
This problem results in a dilemma situation.









% 因此呢 我们认为应当将这个ground to Rec的过程分为两步，第一步是将空间ground，第二步是ground到item
To overcome this problem, we are of the opinion that this process of grounding the LLM to a recommendation ought to be divided into two stages.
% 为了能够将语言简单的转化成真实世界中的item，我们首先要要考虑的是将大模型的输出空间ground到meaningful的item的空间
In the first stage, we should ground the output space of the LLM to the semantic representation space of the actual existing themes in the real world, which could be seen as an abstract grounding stage since we can not ensure the item generated from the semantic representation space is meaningful.
During this stage, we should fully exploit the distinctive advantages of the LLM, enabling the LLM to quickly localize its high-dimensional output space and generate an item from those space.
In the second stage,  we ought to ground the output of the LLM to a real-world item, which is a concrete grounding stage due to each of the items being substantively extant. 
% At this juncture, we ought to utilize the recognization ability  in an expeditious yet accurate manner
At this juncture, due to the LLM generate from a high-dimensional space coming from its understanding of the real world, we ought to utilize its prior knowledge of its cognition of the real world to accomplish this concrete grounding stage in an expeditious yet accurate manner.
%
% 





% 基于大模型在预训练阶段见过丰富的知识，我们认为核心是激发大模型的特定部分的知识，将大模型的输出空间约束到任务特定的空间，就能很好的利用大模型就推荐
%Based on LLMs having witnessed abundant knowledge during the pre-training stage, we opine the crux lies in exciting the specific segments of knowledge within themselves, restricting the output space to a task-specific space, which could sufficiently leverage LLMs for recommendation purposes.
% 为此，我们考虑到大模型是以生成为目的的模型而不是一个discriminator (Yes or No)，因此我们应该尽量减少预训练任务和推荐任务之间存在的gap来帮助我们激发LL预训练阶段学到的知识来执行推荐任务
%For this reason, we should take into consideration that the LLMs are generators rather than discriminators, and thus we ought to minimize the gap between the pre-training process and the recommendation task at hand, so as to optimally harness the knowledge gained in the pre-training stage to effectively discharge the recommendation.
% 总的来说，为了达成这个目标，我们分两阶段来考虑
%In essential terms, to accomplish this objective, we consider \todo{constructing a framework} in two stages:
%1) grounding to the task. 
% 在这个阶段，我们应当充分发挥大模型的特殊优势，让大模型能够快速的定位其对于特定推荐任务的高维输出空间
%During this stage, we should fully exploit the distinctive advantages of the LLM, enabling the LLM to quickly localize its high-dimensional output space for specific recommendation tasks.
%%%%%% 感觉这里要强调出利用大模型的特性，要不然容易被GPT4Rec和抽象feng的GenRec搞到一起 %%%%%
% 2) grounding to the real-world 将大模型在特定输出空间内寻找到的解映射到真实世界中存在的物品上
%2) grounding to the real world.
% 在这个阶段，我们应当考虑对于一个输出空间内的解，简单快速的将其映射到真实世界中存在的item上
%At this juncture, we ought to contemplate a mapping of solutions within the output space to a real-world item in an expeditious yet accurate manner.

% 第四段：为了实现上述目d 标，讲一下简单的思路。提出的简单模型。
% 1）tuning stage: few-shot tuning + title. grounding到推荐任务。
% 2) inference stage: ideal item + rounding. 


% 为了验证我们框架的有效性，我们用一个简单的方法实现了这个框架，同时为了让推荐任务更适配LLM，
In order to test the efficacy of our framework, we realize this framework in a straightforward fashion and customize the recommendation chore to render it more adaptable to the LLM.
In detail, when providing the items a user has interacted with heretofore, we require the LLM to directly generate the next item.
% 我们利用一个少量样本的instruction tuning来完成第一阶段，利用LLM自身的快速alignment能力将LLM grouding到一个具体的task
As for the implementation of the first stage, we apply instruction tuning with few samples to accomplish the first stage, thereby leveraging the intrinsic propensity of LLM for rapid alignment to ground the LLM to a specific task.
% 对于第二阶段，我们简单的利用大模型自身的embedding表示在高维空间中利用L2 Distance进行groud
While for the second stage, we adopt a rudimentary approach by utilizing the latent representations of the LLMs themselves in their high dimensional embedding space via L2 distance as a ground approximation.
% 尽管这仅仅是一个简单的尝试, 但是我们惊讶的发现在相同样本的情况下，他相比于传统方法有着显著的提升，即使和远超其训练数据量的baseline模型相比，仍然保持了comparable的结果
Despite this beginning only a preliminary attempt, we are surprised to discover that, on the equal samples, it shows a significant improvement over traditional recommendation models, retaining comparable results even against baseline models with massively large training data.

% 第五段：实验 + 思考。extension findings。
% Extension: 思考
% 1）LLM4Rec在unpopular item recommendation更友好。
% 2) encoder-decoder和 decoder-only framework上的区别。in recommendation which is better? 

% 在观察到我们的方法的有效性后，我们进一步思考LLM与推荐任务之间的关系
Upon witnessing the effectiveness of our framework, we further contemplate the relation between the LLM and the recommendation task.
% 首先对于LLM来说，由于其在预训练阶段见过很多item，因此在finetuning过程中item出现频次对其的影响相对于传统模型来说理应会更小
% Firstly as far as the LLM is concerned, it has seen many items during its pre-training process, and has acquired specific information about those items.
First of all, for LLM, owing to it having seen a plethora of data during pre-training and learning the semantic associations between that data, the frequency of items occurring during the tuning stage is likely to impact it comparatively less than conventional models.
%因此相比于传统推荐模型来说，他有可能对于训练过程中出现频次不那么高的item更友好, 从另一个角度来说引入一些在grounding to the item阶段引入一些流行度信息可能有助于提升模型的性能
Thus in comparison to traditional recommender models, it could potentially be more amenable to items with lower frequencies during training.
From another perspective, introducing popularity information at the grounding to the item stage may aid in enhancing the model's performance.
% 另一方面来说，目前的LLM主要分为encoder-decoder和decoder两种架构，在推荐领域中哪个更好是一个有待商榷的问题
% Besides, current LLMs are predominantly of the encoder-decoder and decoder architectures; the question as to which is more advantageous in the domain of recommendations remains open to debate.
% 我们认为encoder-decoder架构将输入序列信息整合的过程，一方面需要大量的数据来训练这个特征提取器，另一方面在信息聚合的过程中难免有信息丢失。
% We of the view be that the encoder-decider framework integration process of input sequential information, on the one hand, requires massive data to coach this characteristic extractor, the other side in the aggregation procedure inevitably loses the information.
% 而对于decoder架构来说,在生成的时候可以通过attention细粒度的考量之前的每一个item，因此我们认为decoder架构可能更适用于推荐任务
% Whilst for the decoder framework, we can consider each item previously at a fine-grained level through the attention mechanism, thus we 
% assume that the decoder framework is possibly more suitable for recommendation tasks.
To substantiate the aforementioned hypothesis, we conducted several quantitative analysis experiments, and the experimental findings likewise lent credence to our conjecture.
% 第四段 
% To verify 
% 基于动机1，我们把推荐拟合成一个生成任务，给定用户之前交互的物品直接生成下一个物品的名称，并利用一个简单的基于L2 Distance的方法快速计算物品的All Rank排序
% To validate our assumption, we formulate the sequential recommendation task as a generative task and use only 1024 examples to train the LLM (e.g. LLaMA).
% Specifically, when provided with the items a user has interacted with heretofore, we require the LLM to directly generate the next item, and then we utilize LLM itself to recall the item on the item sets in the dataset.
% Ultimately, we can obtain the performance of the LLMs on the recommendation task in respects of the all-rank performance.
% In practice, we validate the method on two datasets for comparison with the baseline, one of which is dominated by popularity (movie) while the other is not (game).
% We compare our method on the popularity and balanced testset to demonstrate the LLM's advantage for unpopular items, the popularity test set constitutes a typical test set dominated by popularity while the balanced test set comprises a completely balanced test set for each item.
% Moreover, as we previously mentioned, the LLM finds it difficult to receive influence from popularity, thus we introduce popularity information into the LLM's generations in an casual manner in order to further boost the LLM's performance on the popularity dominated dataset.
% 基于动机2，我们在两个数据集上进行验证以对比baseline，其中一个pop占主导，另一个pop不占主导，同时我们还对比了pop和unpop两种测试集来表明大模型对于unpop的物品具有极强的鲁棒性
% 基于动机3，我们提出了一种基于casual的方法，来提升大模型在pop测试集上的能力
% 基于生成动机： 我们做了探索性的扩展实验
% 第五段
% 上述实验结果表明
% 1： 大模型的all rank blablabla
% 2： 大模型在unpop上非常鲁棒，相比传统baseline blabla
% 3： 符合我们的预期 大模型结合pop 在pop占主导的数据上有明显提升，且对参数不敏感
% 4:  扩展实验表明，大模型能够快速学习到相应的能力，生成promising的图片
% Our experiments show that, 
% We conduct our experiments 
% Our experiment results show that, on one hand, with the same amount of training data, the LLM exhibits dominant advantages, with more substantial improvements on the balanced test set compared to the popular test set.
% On the other hand, even when compared to those traditional models trained on full data (8M for movie and 140K for game), the LLM trained only with 1024 samples still show an immense enhancement in the top ranking, demonstrating the reliability of generative recommendation using LLMs.
% Moreover, when we introduce popularity information in a causal manner, we find that it could further boost the recommendation performance on data where popularity dominates, validating our hypothesis.
% In conclusion, our contributions are as follows:
% \begin{itemize}
%     \item We point out that in the recommendation task, we should regard the LLM as a generative model rather than a selection model, which could make fully use of the capability of the LLM.
%     \item We deeply analyze the generative recommendation based on LLM, we indicate that in comparison to the conventional models, the advantages of these models lies in recommendations for unpopular items and their ability to effectively learn recommendation tasks.
%     \item We underscore that the LLM is hard to influence by the popularity information and propose incorporating popularity information into the LLM's recommendations in a casual manner.
% \end{itemize}
In conclusion, our contributions are as follows:
\begin{itemize}
    \item % 我们构建了一个由两阶段grounding构成的全新大模型时代推荐范式，它能够利用大模型的固有的特殊性质快速适配到像all ranking这样的特定推荐任务上。
    We have devised a novel paradigm for LLM recommendations, which comprises a two-stage grounding approach. This approach harnesses the inherent properties of LLMs and enables rapid adaptation to specific recommendation tasks, such as all ranking \todo{The name of paradigm}.
    \item % 基于提出的范式的指导，我们基于大模型的固有特性设计了一个极其简单的方法。实验证明了这个方法的有效性，展示了我们提出的范式的惊人潜力。
    With guidance from the proposed paradigm, we have devised an exceedingly simple approach that leverages the inherent properties of LLMs. Experimental evidence demonstrates the effectiveness of this approach, showcasing the remarkable potential of the paradigm we put forward \todo{The name of paradigm}.
    \item % 我们深入思考了LLM和推荐任务之间的关系，为未来的发展提供了方向。
    We have delved deeply into the correlation between LLM and the recommended task, thereby providing direction for future advancement.
\end{itemize}
% 我们构建了一个


% 第六段
% 我们的contribution
% 1.  指出在推荐任务中，我们应当将大模型作为一个生成模型，而非一个选择模型，以生成为基准的推荐模型拥有更广阔的探索空间，并进行了探索性的尝试
% 2.  通过分析实验表明大模型对于传统推荐的优势在于unpop的集合和其快速学习推荐任务的能力
% 3.  指出大模型难以快速学习到流行度信息，并提出利用casual的方式将流行度信息融入大模型推荐


==> AAintro-backup-0718.tex <==
\section{Introduction}

% Nowadays, Large Language Models (LLMs) exhibit their mighty powers across multiple domains. 
Large Language Models (LLMs) have garnered significant success across various domains \todo{such as XXX and XXX} due to their enormous context comprehension and generation capabilities~\cite{chowdhery2022palm, driess2023palm, wu2023exploring, llm_survey}. 
% In practice, LLMs demonstrate enormous contextual comprehension and generation capabilities, allowing individuals are able to command the LLMs to carry out diverse tasks well via straightforward natural language instructions~\cite{}. 
% Furthermore, different from traditional language models (e.g. BERT~\cite{}, GPT2~\cite{}), researchers have pointed out that LLM possesses the ability to reason based on real-world knowledge and the ability to learn a new task with just a small amount of samples. 
Surpassing traditional language models such as BERT~\cite{bert} and GPT2~\cite{gpt2}, LLMs encode more knowledge, possess mightier reasoning abilities, and can be smoothly adapted to a new task through in-context learning with a few examples~\cite{bao2023tallrec, alpaca}. 
% Currently, in the field of recommendation, studies exploring utilizing LLMs for better recommendations are also developing vigorously~\cite{}. 
In light of this, the exploration of utilizing LLMs for recommendation (LLM4Rec) is evolving vigorously~\cite{wu2023survey, fan2023recommender,FaiRLLM}. 

% Within this important research direction of LLMs for recommendations (LLM4Rec), a valuable issue is, what novel possibilities have LLMs brought to the domain of recommendation and how can we make use of LLMs greatly in the recommendations? 


\begin{figure*}
    \centering
    % \begin{subfigure}
    %     \centering
    %     \includegraphics[width=4cm]{Figure&Table/RQ3_NDCG.pdf}
    %     % \includegraphics[width=4.5cm]{figure.pdf}
    % \end{subfigure}
    % \begin{subfigure}
    %     \centering
    %     \includegraphics[width=4cm]{Figure&Table/RQ3_HR.pdf}
    % \end{subfigure}
    % \caption{This figure displays the improvement in performance after incorporating popularity in the grounding to the real-world stage, as compared to before its inclusion. The left side showcases the NDCG results for varying Top k values, while the right side exhibits the HR results.}
    \includegraphics[width=1\textwidth]{Figure&Table/XRec.pdf}
    \caption{This figure displays the paradigm comprises two grounding steps. During the first step,  %are grounding \zjz{to} abstract spaces, 
    we ground the output space of the model to the semantic representational space of real-world items. While the second stage, we shall ground the outputs generated from sampling the space to a concrete real-world item. }
    % 接下来需要进行的修改：
    % 1. stage 1 中最好能够体现出从output space到 semantic representation space是一个约束的过程，亦即semantic representation space是output space的一个子集。同时最好能体现出可以同时ground多个space
    % 2.stage 2 中生成的item不一定是真实世界有的，亦即不是generated item就是real world item，我们其实是在找到和这个generated item最接近的real world item来进行grounding。
    
    \label{fig:paradigm}
\end{figure*}

% In recent attempts, there have been a lot of works aimed at introducing LLMs into recommendations, which principally break into two groups -- In-context Learning based and Instruction-tuning based~\cite{wu2023survey}.
Recent work on LLM4Rec principally falls into two groups -- \textit{in-context learning-based} and \textit{instruction tuning-based} methods~\cite{wu2023survey}. 
% todo: 统一这两个term的格式，应该不用首字母大写，instruction tuning 谷歌的论文里好像也没有- 
% For the former, they attempt to call an accessible API (e.g. ChatGPT), and by giving the model several recommendation examples request the LLM to conduct recommendatoins~\cite{}. 
In-context learning-based methods instruct LLMs to generate recommendations by providing several recommendation examples in the prompts~\cite{liu2023chatgpt}. 
% Yet owing to the fact that there exists a gap between the pre-training task of LLms and the recommendations, the LLM lacks domain-specific recommendation knowledge, which is hard to eliminate this gap through a simple prompt, eventually resulting in an inferior performance. 
% Yet owing to the significant gap between the pre-training tasks of LLMs and the recommendation task, LLMs lack sufficient recommendation knowledge. Instructing LLM4Rec with several examples eventually results in poor recommendation performance. 
Yet in-context learning-based LLM4Rec eventually results in poor performance owing to the significant gap between the pre-training tasks of LLMs and the recommendation task~\cite{bao2023tallrec, zhang2023recommendation}.
% For the latter, researchers try to teach the LLM how to recommend through instruction tuning and get a promising result~\cite{bao2023tallrec}.
By contrast, instruction tuning-based methods aim to reduce the gap by fine-tuning LLMs with recommendation data~\cite{bao2023tallrec, zhang2023recommendation}.
% However, current models only show a limited recommendation performance.
Nevertheless, existing fine-tuning methods still \todo{suffer from an inferior performance} than traditional recommender models in most recommendation settings~\cite{xxx}. % todo: add a reference and check whether this claim is dangerous. 
% todo: most recommendation settings. need to revise this. XXX setting? 具体到某种推荐settings？
% Additionally, current researchers often delimit the range of items visible to the model which is difficult to show the real performance of the recommendation ability of LLMs. 
% As such, 
% what novel possibilities have LLMs brought to the domain of recommendation and how can we make use of LLMs greatly in the recommendations? 

% In general, we attribute this inferior performance to their disagreement between the pre-training phase and the instruction-tuning phase.
In general, we attribute this \todo{inferior performance} to the disagreement between the instruction tuning and the pre-training of LLMs. 
% Question: 需要回答一个问题，二者怎么disagree了？换句话说，这是怎样的disagreement
During the pre-training stage, LLMs predict the next token freely in a generative manner. However, previous LLM4Rec usually fine-tunes LLMs via discriminative tasks, \eg judging whether a user would like an item~\cite{bao2023tallrec} or \todo{predicting the ranking of item candidates}~\cite{zhang2023recommendation}. 
% \todo{usually XXX or restrict the outputs of LLMs to existing item indexes (\eg IDs or XXX) by XXX (beam search or others?)}. 
% Question: 上面论证existing LLM4Rec咋就没消除disagreement。
% disagreement的后果：
Such a disagreement undermines the generative capabilities of LLMs and hampers the comprehensive utilization of the pre-training knowledge of LLMs. 
% todo: 修改后果这句话。这样的disagreement or restriction为什么会导致performance变差。
As such, to fully exploit LLMs for the recommendation, we consider addressing the disagreement and unleashing the powerful generative capabilities of LLMs. 
% Therefore, we should be in consonance with the training mode of the pre-training stage and employ a generative modality that directly yields the next item to minimize this gap to assist us in better utilizing LLM to the recommendation.
% In other words, we ought to ground the LLM to the recommendation, by transferring the output of the LLM to a meaningful item in the real world for recommendation. 
% However, owing to the creative generative capabilities of the LLM, directly restricting the generated outputs to a specific item set is a difficult task; moreover, overly restricting the model outputs means that it will struggle to adapt to a novel item, even though the LLM recognizes it. 
% This problem results in a dilemma situation.


%%% keqin: 为啥一定要两个阶段，一个阶段不行
% 一方面由于LLM生成的创造性，因此我们很难保证LLM生成的结果一定有真实意义，一定生成存在的item
% 另一方面如果我们限制死LLM的生成结果（保证生成一定在范围内），这就导致LLM很难适配新的item，即使这个item的知识LLM知道，由于生成结果被限制死了，我们也不能利用这个系统进行推荐
To harness the generative capabilities of LLMs for the recommendation, the key lies in alleviating a dilemma --- the generated output of LLMs might lack meaningful correspondence with real-world items; restricting the outputs of LLMs to existing \todo{item representations} (\eg IDs or titles)
will fall short in recommending unseen items during instruction tuning.
% , they will fall short in recommending cold-start items (which are \bkq{unseen} during the instruction tuning stage). 
In light of this, 
\bkq{To alleviate this issue, we develop a grounding paradigm for LLM-based recommendation with two grounding steps.}
First, given the instruction input of the recommendation task (\eg task instruction and user interaction history), LLMs should be grounded \bkq{in order to} freely generate tokens for the next item prediction, \ie LLMs ought to be aware of the semantic generation space for the recommendation as shown in Figure~\ref{fig:paradigm}. % 增加一个图来解释？ // 
% 这一段，说实话我没想好咋写更好，可能配合一个图来讲会好一些，没那么抽象，要不然太抽象了，很难让人读懂。我觉得之前那段应该是八成的人读不懂的。
Second, the generated tokens should be grounded to adapt to real-world items for recommendations. 
% Question: 这两个grounding steps怎么就能够缓解disagreement的问题了？，since we attribute this inferior performance to the disagreement between the instruction tuning and the pre-training of LLMs. 
% answer: 
% Intuitively, based on the instruction input, LLMs can generate an ``ideal'' item that the user might like. 
% This process aligns well with the pre-training of LLMs in a generative manner. 
% In the second stage, the ``ideal'' item ought to be grounded to a real-world item for a recommendation. 




% To overcome this problem, we are of the opinion that this process of grounding the LLM to a recommendation ought to be divided into two stages. 
% In the first stage, we should ground the output space of the LLM to the semantic representation space of the actual existing themes in the real world, which could be seen as an abstract grounding stage since we can not ensure the item generated from the semantic representation space is meaningful. 
% During this stage, we should fully exploit the distinctive advantages of the LLM, enabling the LLM to quickly localize its high-dimensional output space and generate an item from those space.
% In the second stage,  we ought to ground the output of the LLM to a real-world item, which is a concrete grounding stage due to each of the items being substantively extant. 
% At this juncture, due to the LLM generate from a high-dimensional space coming from its understanding of the real world, we ought to utilize its prior knowledge of its cognition of the real world to accomplish this concrete grounding stage in an expeditious yet accurate manner. 



To understand the potential of our paradigm, we develop a simple \underline{g}r\underline{o}unding \underline{a}pproach for \underline{L}LM-based \underline{rec}ommendations (GoalRec) to conduct an in-depth analysis of it. 
In practice, in the first step, we construct the recommendation task instruction and users' interacted item histories as the instruction input and tune the LLMs to generate the title of the target item (see Table~\ref{tab:example}). 
By this instruction tuning with few samples, LLMs can be grounded to be aware of \bkq{the representation space of the candidate items for the recommendation task}. 
And during the inference phase, given an instruction input, LLMs can freely generate a list of tokens, which represent an ``ideal'' item that the user might like. 
\zjz{For the second step}, the ``ideal'' item ought to be grounded to a real-world item as a recommendation. 
To achieve this, we adopt LLMs to extract latent representations of the ``ideal'' item and the real-world items, and then locate the most matched real-world items via L2 distance for recommendations. 
% todo: 检查我写的implementation有没有逻辑问题？ ok

We conduct extensive experiments on two real-world datasets with various settings, for instance, 
% \bkq{
% First, we compare the performance of our model and traditional recommender models on the same number of samples, and the results show that our model achieved breathtaking superiority.
% Besides, we also testify the traditional recommender models with more samples (over 7M for Movies and 120K for Games), even when we only used 1024 samples, our model maintained competitiveness in most cases with the traditional recommender models.
% Moreover, we find that the LLM can easily ground their output space to different representation space simultaneously (\ie Movies and Games' candidate items). 
% } 
\todo{few-shot and full-data training settings} (refer to Section~\ref{section:exp}).
% 可以再修改一下这两个的名字，intro没有太多空间写这么细的setting介绍。
The empirical results show that our method surpasses traditional recommender models and existing LLM4Rec methods under few-short training. Furthermore, with few-shot training ($\sim 1k$ samples) surprisingly achieves better or comparable performance than traditional recommender models with full training \bkq{($\sim 7M~and~120K$ samples for two datasets, respectively)}. 
% todo: 讲一下few-shot 以及不同的比较的settings。
% 目前是在Movie和Games数据集上都few-shot比较，并进行了分析 结果高很多（感觉这个比较正常）
% 在Movie和Games上用few-shot的结果比较了SASRec Caser GRU4Rec full-training （Movie: 7.4M数据，Games 120K）的结果 （这个结果更有说服力一点）
% 另外我们做了实验表明，我们可以同步grounding多个空间 (e.g. 可以同时将Movie对应的输出到Movie Item的空间，Games对应的输出到Game Item的空间）
% The empirical results validate the superiority of XXX over traditional recommender models and existing LLM4Rec methods. 
% Upon witnessing the effectiveness of GoalRec, 
We further discuss the two additional findings from the investigations of LLM4Rec. 
% First of all, for LLM, owing to it having seen a plethora of data during pre-training and learning the semantic associations between that data, the frequency of items occurring during the tuning stage is likely to impact it comparatively less than conventional models. 
% Thus in comparison to traditional recommender models, it could potentially be more amenable to items with lower frequencies during training. 
First, compared to conventional recommender models, LLM4Rec is potentially more friendly to sparse items with low frequencies in the instruction tuning data. 
This is because a plethora of data is used for pre-training LLMs, and thus the item frequency in the instruction tuning data is likely to reveal a smaller impact on LLMs. 
% From another perspective, introducing popularity information at the grounding to the item stage may aid in enhancing the model's performance. 
Besides, introducing items' popularity information to the item grounding stage can significantly enhance the model performance. 
% To substantiate the aforementioned hypothesis, we conducted several quantitative analysis experiments, and the experimental findings likewise lent credence to our conjecture. 

In conclusion, our contributions are as follows:
\begin{itemize}[leftmargin=*]
    \item 
    % We have devised a novel paradigm for LLM recommendations, which comprises a two-stage grounding approach. This approach harnesses the inherent properties of LLMs and enables rapid adaptation to specific recommendation tasks, such as all ranking \todo{The name of paradigm}. 
    We propose \bkq{a grounding paradigm}, which unleashes the generative capabilities of LLMs and \bkq{convenient insertion of information that benefits recommendations.}
    % \todo{enables rapid adaptation to recommendation tasks. }
    \item 
    % With guidance from the proposed paradigm, we have devised an exceedingly simple approach that leverages the inherent properties of LLMs. Experimental evidence demonstrates the effectiveness of this approach, showcasing the remarkable potential of the paradigm we put forward \todo{The name of paradigm}.
    We develop an exceedingly simple approach for our grounding paradigm, namely GoalRec, which grounds the outputs of LLMs for recommendation through two \bkq{steps}. 

    \item Experimental evidence demonstrates the effectiveness of GoalRec, showcasing the remarkable potential of our grounding paradigm.
    
    \item 
    % We have delved deeply into the correlation between LLM and the recommended task, thereby providing direction for future advancement. 
    We deeply discuss the benefits of \bkq{our paradigm} and point out some promising research directions, facilitating future advancement in this booming field. 
    
\end{itemize}


==> AAintroduction-backup-0726.tex <==
\section{Introduction}
Large Language Models (LLMs) have garnered significant success across various domains (such as CV and Robotics) due to their enormous context comprehension and generation capabilities~\cite{chowdhery2022palm, driess2023palm,  llm_survey}. 
Surpassing traditional language models such as BERT~\cite{bert} and GPT2~\cite{gpt2}, LLMs encode more knowledge, possess mightier reasoning abilities, and can be smoothly adapted to a new task through in-context learning with a few examples~\cite{bao2023tallrec, alpaca, chatgpt_mol}. 
In light of this, the exploration of utilizing LLMs for recommendation (LLM4Rec) is evolving vigorously~\cite{wu2023survey, fan2023recommender,FaiRLLM,IR_report}. 

\input{Figure&Table/Fig1}

% In recent attempts, there have been a lot of works aimed at introducing LLMs into recommendations, which principally break into two groups -- In-context Learning based and Instruction-tuning based~\cite{wu2023survey}.
Recent work on LLM4Rec principally falls into two groups -- \textit{in-context learning-based} and \textit{instruction tuning-based} methods~\cite{wu2023survey}. 
% todo: 统一这两个term的格式，应该不用首字母大写，instruction tuning 谷歌的论文里好像也没有- 
% For the former, they attempt to call an accessible API (e.g. ChatGPT), and by giving the model several recommendation examples request the LLM to conduct recommendatoins~\cite{}. 
In-context learning-based methods instruct LLMs to generate recommendations by providing several recommendation examples in the prompts~\cite{liu2023chatgpt}. 
% Yet owing to the fact that there exists a gap between the pre-training task of LLms and the recommendations, the LLM lacks domain-specific recommendation knowledge, which is hard to eliminate this gap through a simple prompt, eventually resulting in an inferior performance. 
% Yet owing to the significant gap between the pre-training tasks of LLMs and the recommendation task, LLMs lack sufficient recommendation knowledge. Instructing LLM4Rec with several examples eventually results in poor recommendation performance. 
Yet in-context learning-based LLM4Rec eventually results in poor performance owing to the significant gap between the pre-training tasks of LLMs and the recommendation task~\cite{bao2023tallrec, zhang2023recommendation}.
% For the latter, researchers try to teach the LLM how to recommend through instruction tuning and get a promising result~\cite{bao2023tallrec}.
By contrast, instruction tuning-based methods aim to reduce the gap by fine-tuning LLMs with recommendation data~\cite{bao2023tallrec, zhang2023recommendation}.
% However, current models only show a limited recommendation performance.
Nevertheless, existing fine-tuning methods still suffer from an inferior performance (refer to Section~\ref{section:exp}) than traditional recommender models in most recommendation settings. 
% 
% todo: add a reference and check whether this claim is dangerous. 
% todo: most recommendation settings. need to revise this. XXX setting? 具体到某种推荐settings？
% Additionally, current researchers often delimit the range of items visible to the model which is difficult to show the real performance of the recommendation ability of LLMs. 
% As such, 
% what novel possibilities have LLMs brought to the domain of recommendation and how can we make use of LLMs greatly in the recommendations? 

In general, we attribute this inferior performance to the disagreement between the instruction tuning and the pre-training of LLMs. 
% Question: 需要回答一个问题，二者怎么disagree了？换句话说，这是怎样的disagreement
During the pre-training stage, LLMs predict the next token freely in a generative manner. However, previous LLM4Rec usually fine-tunes LLMs via discriminative tasks, \eg judging whether a user would like a \zjz{given} item~\cite{bao2023tallrec} or predicting the ranking of \zjz{the given item candidates in the prompt}~\cite{zhang2023recommendation}. 
% \todo{usually XXX or restrict the outputs of LLMs to existing item indexes (\eg IDs or XXX) by XXX (beam search or others?)}. 
% Question: 上面论证existing LLM4Rec咋就没消除disagreement。
% disagreement的后果：
Such a disagreement undermines the generative capabilities of LLMs and hampers the comprehensive utilization of the pre-training knowledge of LLMs. 
% todo: 修改后果这句话。这样的disagreement or restriction为什么会导致performance变差。
As such, to fully exploit LLMs for the recommendation, we consider addressing the disagreement and unleashing the powerful generative capabilities of LLMs. 
% Therefore, we should be in consonance with the training mode of the pre-training stage and employ a generative modality that directly yields the next item to minimize this gap to assist us in better utilizing LLM to the recommendation.
% In other words, we ought to ground the LLM to the recommendation, by transferring the output of the LLM to a meaningful item in the real world for recommendation. 
% However, owing to the creative generative capabilities of the LLM, directly restricting the generated outputs to a specific item set is a difficult task; moreover, overly restricting the model outputs means that it will struggle to adapt to a novel item, even though the LLM recognizes it. 
% This problem results in a dilemma situation.


%%% keqin: 为啥一定要两个阶段，一个阶段不行
% 一方面由于LLM生成的创造性，因此我们很难保证LLM生成的结果一定有真实意义，一定生成存在的item
% 另一方面如果我们限制死LLM的生成结果（保证生成一定在范围内），这就导致LLM很难适配新的item，即使这个item的知识LLM知道，由于生成结果被限制死了，我们也不能利用这个系统进行推荐
To harness the generative capabilities of LLMs for recommendation, the key lies in grounding the output of the LLM to recommend real-world items. 
Directly matching the generated output of LLMs with real-world items or restricting the LLM to generate items are seemingly feasible solutions.
However, the output of LLMs might lack meaningful correspondence with real-world items; restricting the LLM to generate existing items (\eg IDs) will fall short of recommending unseen items.
In light of this, we formulate a two-step grounding paradigm with language space $\rightarrow$ recommendation space $\rightarrow$ real-world item space as shown in Figure~\ref{fig:paradigm}, where the \bkq{language space contains all possible sequences LLM can generate}, and recommendation space is the sub-space of the language space which describes \bkq{all possible items including both real items and imaginary items might satisfy user needs}. 
In particular, the first step grounds LLMs to the recommendation space in order to generate meaningful tokens for describing the item; % 增加一个图来解释？ // 
% 这一段，说实话我没想好咋写更好，可能配合一个图来讲会好一些，没那么抽象，要不然太抽象了，很难让人读懂。我觉得之前那段应该是八成的人读不懂的。
the second step grounds the generated tokens to real-world item space for recommendations. 
% Question: 这两个grounding steps怎么就能够缓解disagreement的问题了？，since we attribute this inferior performance to the disagreement between the instruction tuning and the pre-training of LLMs. 
% answer: 
% Intuitively, based on the instruction input, LLMs can generate an ``ideal'' item that the user might like. 
% This process aligns well with the pre-training of LLMs in a generative manner. 
% In the second stage, the ``ideal'' item ought to be grounded to a real-world item for a recommendation. 




% To overcome this problem, we are of the opinion that this process of grounding the LLM to a recommendation ought to be divided into two stages. 
% In the first stage, we should ground the output space of the LLM to the semantic representation space of the actual existing themes in the real world, which could be seen as an abstract grounding stage since we can not ensure the item generated from the semantic representation space is meaningful. 
% During this stage, we should fully exploit the distinctive advantages of the LLM, enabling the LLM to quickly localize its high-dimensional output space and generate an item from those space.
% In the second stage,  we ought to ground the output of the LLM to a real-world item, which is a concrete grounding stage due to each of the items being substantively extant. 
% At this juncture, due to the LLM generate from a high-dimensional space coming from its understanding of the real world, we ought to utilize its prior knowledge of its cognition of the real world to accomplish this concrete grounding stage in an expeditious yet accurate manner. 



We further develop a simple \underline{g}r\underline{o}unding \underline{a}pproach for \underline{L}LM-based \underline{rec}ommendations (GoalRec). 
In the first grounding step, we tune the LLM to freely generate a list of tokens, which represent an ``ideal'' item that the user might like. We construct the recommendation task instruction and users' interacted item histories as the instruction input and tune the LLMs to generate the title of the target item (see Table~\ref{tab:example}). 
In the second grounding step, we adopt the LLM to extract latent representations of the ``ideal'' item and real-world items, and then locate the most matched real-world items via L2 distance for recommendations. 

We conduct extensive experiments on two real-world datasets with various settings, for instance, 
% \bkq{
% First, we compare the performance of our model and traditional recommender models on the same number of samples, and the results show that our model achieved breathtaking superiority.
% Besides, we also testify the traditional recommender models with more samples (over 7M for Movies and 120K for Games), even when we only used 1024 samples, our model maintained competitiveness in most cases with the traditional recommender models.
% Moreover, we find that the LLM can easily ground their output space to different representation space simultaneously (\ie Movies and Games' candidate items). 
% } 
few-shot and full-data training settings (refer to Section~\ref{section:exp}).
% 可以再修改一下这两个的名字，intro没有太多空间写这么细的setting介绍。
The empirical results show that our GoalRec surpasses traditional recommender models and existing LLM4Rec methods under few-shot training. Furthermore, GoalRec with few-shot training ($\sim 1k$ samples) surprisingly achieves better or comparable performance than traditional recommender models with full-data training ($\sim7M$ and $\sim120K$ samples for two datasets, respectively). 
% todo: 讲一下few-shot 以及不同的比较的settings。
% 目前是在Movie和Games数据集上都few-shot比较，并进行了分析 结果高很多（感觉这个比较正常）
% 在Movie和Games上用few-shot的结果比较了SASRec Caser GRU4Rec full-training （Movie: 7.4M数据，Games 120K）的结果 （这个结果更有说服力一点）
% 另外我们做了实验表明，我们可以同步grounding多个空间 (e.g. 可以同时将Movie对应的输出到Movie Item的空间，Games对应的输出到Game Item的空间）
% The empirical results validate the superiority of XXX over traditional recommender models and existing LLM4Rec methods. 
% Upon witnessing the effectiveness of GoalRec, 
We further discuss the two additional findings from the investigations of LLM4Rec. 
% First of all, for LLM, owing to it having seen a plethora of data during pre-training and learning the semantic associations between that data, the frequency of items occurring during the tuning stage is likely to impact it comparatively less than conventional models. 
% Thus in comparison to traditional recommender models, it could potentially be more amenable to items with lower frequencies during training. 
First, compared to conventional recommender models, \bkq{LLM} is potentially more friendly to \zjz{unpopular} items with low frequencies in the instruction tuning data. 
This is because a plethora of data is used for pre-training LLMs, and thus the item frequency in the instruction tuning data is likely to reveal a smaller impact on LLMs. 
% From another perspective, introducing popularity information at the grounding to the item stage may aid in enhancing the model's performance. 
Besides, introducing items' popularity information to the item grounding stage can significantly enhance the model performance. 
% To substantiate the aforementioned hypothesis, we conducted several quantitative analysis experiments, and the experimental findings likewise lent credence to our conjecture. 

In conclusion, our contributions are as follows:
\begin{itemize}[leftmargin=*]
    % \item
    % We propose \bkq{a grounding paradigm}, which unleashes the generative capabilities of LLMs and \bkq{convenient insertion of information that benefits recommendations.}

    % \item 
    % We develop an exceedingly simple approach for our grounding paradigm, namely GoalRec, which grounds the outputs of LLMs for recommendation through two \bkq{steps}. 

    \item \bkq{We formulate a grounding paradigm and implement it with a simple approach, which grounds the LLM to recommend real-world items via two steps.}

    \item Experimental evidence demonstrates the effectiveness of our paradigm, showcasing the remarkable potential of our grounding paradigm.
    
    \item 
    % We have delved deeply into the correlation between LLM and the recommended task, thereby providing direction for future advancement. 
    We deeply discuss the benefits of \bkq{our paradigm} and point out some promising research directions, facilitating future advancement in this booming field. 
    
\end{itemize}


==> Figure_Table/RQ4_backup.tex <==

\begin{figure*}[htbp] %通栏
\footnotesize
\begin{minipage}[t]{0.22\linewidth} %调节两个子图左右间距
\centering
\includegraphics[width=1.5in, height=1.4in]{Figure&Table/RQ4_NDCG_movie.pdf} %调节单个子图大小
\end{minipage}%
\begin{minipage}[t]{0.22\linewidth}
\centering
\includegraphics[width=1.5in, height=1.4in]{Figure&Table/RQ4_HR_movie.pdf}
\end{minipage}%
\begin{minipage}[t]{0.22\linewidth}
\centering
\includegraphics[width=1.5in, height=1.4in]{Figure&Table/RQ4_NDCG_games.pdf}
\end{minipage}
\begin{minipage}[t]{0.22\linewidth}
\centering
\includegraphics[width=1.5in, height=1.4in]{Figure&Table/RQ4_HR_games.pdf}
\end{minipage}%
\caption{
Performance comparison of BIGRec trained with multiple spaces data (labeled as `Multiple') and BIGRec trained with single target-domain data (labeled as `Single'), displayed for Movie and Game domains, with left two figures showing Movie results and right two figures showing Games results.
% Multi-domain Results of Proposed Method on Movie and Games Datasets Displayed in Four Figures. Left Bars Represent Results of Single-Domain Training and Testing, while Right Bars Show Results of Joint Training on Both Datasets and Testing on Each Individually
% These four figures demonstrate the multi-domain results of our proposed method on the Movie and Games datasets. 
% The left bars in each column indicate the results of training and testing on a single domain, while the right bars indicate the results obtained by training on both the movie and games datasets, and subsequently testing on each dataset individually.
% The two figures on the left represent the results on the movie dataset, while the two figures on the right represent the results on the games dataset. 
}
\label{fig:multi_domain_result}
\end{figure*}



==> Figure_Table/tab1_underline_backup_1.tex <==
\begin{table*}[]
\centering
\caption{
%This table displays the results of training on 1024 randomly selected sequences from the training set, followed by testing performance on a randomly sampled test set. \textbf{Bold} indicates the best result, while "Improve" represents the improvement of our proposed method relative to the best result obtained using traditional models. N means NDCG and R means HR. 
Comparison of model performances under the few-shot training (1024 samples) with NDCG@K (NG@K) and HR@K (HR@K) as metrics. The best results are highlighted in bold, and the sub-optimal results are underlined. “Improve” refers to the relative improvement of GoalRec over the best baseline.
}
\label{tab:pop_1024}
\resizebox{0.98\textwidth}{!}{
\begin{tabular}{cccccccccccc}
\hline
                        & Model                                        & NG@1                                        & NG@3                                        & NG@5                                       & NG@10                                      & NG@20                                      & HR@1                                        & HR@3                                        & HR@5                                       & HR@10                                      & HR@20                                      \\ \cline{1-12}
                        & GRU4Rec                                      & 0.0015                                     & 0.0034                                     & 0.0047                                    & 0.0070                                    & 0.0104                                    & 0.0015                                     & 0.0047                                     & 0.0079                                    & 0.0147                                    & 0.0281                                    \\
                        & Caser                                        & 0.0020                                     & 0.0035                                     & 0.0052                                    & \underline{0.0078}                                    & \underline{0.0109}                                    & 0.0020                                     & 0.0046                                     & 0.0088                                    & \underline{0.0171}                                    & \underline{0.0293}                                    \\ 
                        & SASRec                                       & \underline{0.0025}                                     & \underline{0.0045}                                     & \underline{0.0057}                                    & 0.0078                                    & 0.0100                                    & \underline{0.0025}                                     & \underline{0.0060}                                     & \underline{0.0090}                                    & 0.0155                                    & 0.0245                                    \\
                        & GPT4Rec-LLaMA & 0.0016 & 0.0022 & 0.0024 & 0.0028 & 0.0035 & 0.0016 & 0.0026 & 0.0030 & 0.0044 & 0.0074 \\
                        & Flan-T5 & 0.0000 & 0.0000 & 0.0001 & 0.0002 & 0.0012  & 0.0000 & 0.0000 & 0.0002 & 0.0006 & 0.0044 \\
                        \cline{2-12} 
                        & \cellcolor[HTML]{EFEFEF}\textbf{GoalRec (Ours)} & \cellcolor[HTML]{EFEFEF}\textbf{0.0182}    & \cellcolor[HTML]{EFEFEF}\textbf{0.0219}    & \cellcolor[HTML]{EFEFEF}\textbf{0.0235}   & \cellcolor[HTML]{EFEFEF}\textbf{0.0262}   & \cellcolor[HTML]{EFEFEF}\textbf{0.0287}   & \cellcolor[HTML]{EFEFEF}\textbf{0.0182}    & \cellcolor[HTML]{EFEFEF}\textbf{0.0247}    & \cellcolor[HTML]{EFEFEF}\textbf{0.0284}   & \cellcolor[HTML]{EFEFEF}\textbf{0.0369}   & \cellcolor[HTML]{EFEFEF}\textbf{0.0471}   \\
\multirow{-5}{*}{Movie} & \cellcolor[HTML]{D0D0D0}\textbf{Improve}     & \cellcolor[HTML]{D0D0D0}\textbf{618.42\%}  & \cellcolor[HTML]{D0D0D0}\textbf{388.31\%}  & \cellcolor[HTML]{D0D0D0}\textbf{312.21\%} & \cellcolor[HTML]{D0D0D0}\textbf{234.41\%} & \cellcolor[HTML]{D0D0D0}\textbf{162.39\%} & \cellcolor[HTML]{D0D0D0}\textbf{618.42\%}  & \cellcolor[HTML]{D0D0D0}\textbf{311.67\%}  & \cellcolor[HTML]{D0D0D0}\textbf{215.56\%} & \cellcolor[HTML]{D0D0D0}\textbf{116.21\%} & \cellcolor[HTML]{D0D0D0}\textbf{60.57\%}  \\ \hline
                        & GRU4Rec                                      & \underline{0.0013}                                     & \underline{0.0016}                                     & 0.0018                                   & \underline{0.0024}                                    & 0.0030                                    & \underline{0.0013}                                     & \underline{0.0018}                                     & 0.0024                                    & 0.0041                                    & 0.0069                                    \\
                        & Caser                                        & 0.0007                                     & 0.0012                                     & \underline{0.0019}                                    & \underline{0.0024}                                    & \underline{0.0035}                                    & 0.0007                                     & 0.0016                                     & \underline{0.0032}                                    & \underline{0.0048}                                    & \underline{0.0092}                                    \\
                        & SASRec                                       & 0.0006                                     & 0.0009                                     & 0.0011                                    & 0.0016                                    & 0.0022                                    & 0.0006                                     & 0.0011                                     & 0.0016                                    & 0.0031                                    & 0.0056                                    \\
                        & GPT4Rec-LLaMA & 0.0000 & 0.0000 & 0.0000 & 0.0001 & 0.0001 & 0.0000 & 0.0000 & 0.0000 & 0.0002 & 0.0002 \\
                        & Flan-T5 & 0.0000 & 0.0000 & 0.0000 & 0.0000 & 0.0001 & 0.0000 & 0.0000 & 0.0000 & 0.0000 & 0.0002 \\
                        & \cellcolor[HTML]{EFEFEF}\textbf{GoalRec (Ours)} & \cellcolor[HTML]{EFEFEF}\textbf{0.0141}    & \cellcolor[HTML]{EFEFEF}\textbf{0.018}     & \cellcolor[HTML]{EFEFEF}\textbf{0.0202}   & \cellcolor[HTML]{EFEFEF}\textbf{0.0225}   & \cellcolor[HTML]{EFEFEF}\textbf{0.0259}   & \cellcolor[HTML]{EFEFEF}\textbf{0.0141}    & \cellcolor[HTML]{EFEFEF}\textbf{0.0209}    & \cellcolor[HTML]{EFEFEF}\textbf{0.0261}   & \cellcolor[HTML]{EFEFEF}\textbf{0.0333}   & \cellcolor[HTML]{EFEFEF}\textbf{0.0468}   \\
\multirow{-5}{*}{Games} & \cellcolor[HTML]{D0D0D0}\textbf{Improve}     & \cellcolor[HTML]{D0D0D0}\textbf{1015.79\%} & \cellcolor[HTML]{D0D0D0}\textbf{1050.40\%} & \cellcolor[HTML]{D0D0D0}\textbf{958.43\%} & \cellcolor[HTML]{D0D0D0}\textbf{835.90\%} & \cellcolor[HTML]{D0D0D0}\textbf{644.53\%} & \cellcolor[HTML]{D0D0D0}\textbf{1015.79\%} & \cellcolor[HTML]{D0D0D0}\textbf{1059.26\%} & \cellcolor[HTML]{D0D0D0}\textbf{716.67\%} & \cellcolor[HTML]{D0D0D0}\textbf{593.06\%} & \cellcolor[HTML]{D0D0D0}\textbf{408.70\%} \\ \hline
\end{tabular}}
\end{table*}

==> Figure_Table/tab2.tex <==
\begin{table*}[]
\caption{
% The presented table showcases the performance outcomes obtained by testing on the balance test set subsequent to training with 1024 randomly chosen sequences from the training set. The entries that are bolded denote the most superior results, whereas the term "Improve" signifies the relative enhancement of the proposed method in comparison to the optimal results achieved by conventional models.
Performance of compared methods on balanced testing sets under the few-show training setting (1024 samples). The best results are highlighted in bold, and the sub-optimal results are underlined. `Improve' refers to the relative improvement of BIGRec over the best baseline.
% after Training with 1024 Random Sequences from Training Set. Bold Entries Indicate Best Results, 'Improve' Signifies Relative Enhancement of Proposed Method over Conventional Models.
}
\label{tab:unpop_1024}
\resizebox{0.98\textwidth}{!}{
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}
\begin{tabular}{cccccccccccc}
\hline
                        & Model                                        & NG@1                                        & NG@3                                        & NG@5                                       & NG@10                                      & NG@20                                      & HR@1                                        & HR@3                                        & HR@5                                       & HR@10                                      & HR@20                                                \\ \hline
                        & GRU4Rec                                      & 0.00010                                    & 0.00021                                    & 0.00029                                    & {0.00046}                                    & 0.00071                                    & 0.00010                                    & {0.00030}                                    & {0.00050}                                    & {0.00102}                                    & {0.00205}                                    \\
                        & Caser                                        & 0.00010                                    & 0.00021                                    & 0.00029                                    & {0.00046}                                    & {0.00071}                                    & 0.00010                                    & {0.00030}                                    & {0.00050}                                    & {0.00102}                                    & 0.00202                                    \\
                        & SASRec                                       & {0.00013}                                    & {0.00022}                                    & {0.00030}                                     & {0.00046}                                    & 0.00071                                    & {0.00013}                                    & {0.00030}                                    & {0.00050}                                    & 0.00099                                    & 0.00198                                    \\ 
                        & GPT4Rec-LLaMA & 0.00010 & 0.00021 & 0.00029 & 0.00045 & 0.00070 & 0.00010 & {0.00030} & {0.00050} & 0.00099 & 0.00198 \\
                         & DROS & 0.00013&	0.00023&	0.00031&	0.00046&	0.00071&	0.00013&	0.00030&	0.00050&	0.00096&	0.00195 \\
                         & P5 &0.00026&	0.00046&	0.00061&	0.00084&	0.00110&	0.00026&	0.00059&	0.00096&	0.00169&	0.00271 \\
                        \cline{2-12}
                        
                        & \cellcolor[HTML]{EFEFEF}\textbf{BIGRec (1024)} & \cellcolor[HTML]{EFEFEF}\textbf{0.00595}   & \cellcolor[HTML]{EFEFEF}\textbf{0.00694}   & \cellcolor[HTML]{EFEFEF}\textbf{0.00753}   & \cellcolor[HTML]{EFEFEF}\textbf{0.00836}   & \cellcolor[HTML]{EFEFEF}\textbf{0.00921}   & \cellcolor[HTML]{EFEFEF}\textbf{0.00595}   & \cellcolor[HTML]{EFEFEF}\textbf{0.00767}   & \cellcolor[HTML]{EFEFEF}\textbf{0.00909}   & \cellcolor[HTML]{EFEFEF}\textbf{0.01167}   & \cellcolor[HTML]{EFEFEF}\textbf{0.01514}   \\
                        								
\multirow{-7}{*}{Movie} & \cellcolor[HTML]{D0D0D0}\textbf{Improve}     & \cellcolor[HTML]{D0D0D0}\textbf{3500.00\%} & \cellcolor[HTML]{D0D0D0}\textbf{1719.10\%} & \cellcolor[HTML]{D0D0D0}\textbf{1518.18\%} & \cellcolor[HTML]{D0D0D0}\textbf{1267.62\%} & \cellcolor[HTML]{D0D0D0}\textbf{986.58\%} & \cellcolor[HTML]{D0D0D0}\textbf{3500.00\%} & \cellcolor[HTML]{D0D0D0}\textbf{1350.00\%} & \cellcolor[HTML]{D0D0D0}\textbf{1150.00\%} & \cellcolor[HTML]{D0D0D0}\textbf{880.56\%} & \cellcolor[HTML]{D0D0D0}\textbf{615.62\%}  \\ \hline
                        & GRU4Rec                                      & {0.00012}                                    & 0.00034                                    & {0.00043}                                    & 0.00064                                    & 0.00092                                    & {0.00012}                                    & 0.00048                                    & {0.00071}                                    & 0.00137                                    & 0.00250                                    \\
                        & Caser                                        & {0.00012}                                    & {0.00036}                                    & {0.00043}                                    & {0.00066}                                    & {0.00098}                                    & {0.00012}                                    & {0.00054}                                    & {0.00071}                                    & {0.00143}                                    & {0.00274}                                    \\
                        & SASRec                                       & {0.00012}                                    & 0.00026                                    & 0.00041                                    & 0.00060                                     & 0.00084                                    & {0.00012}                                    & 0.00036                                    & {0.00071}                                    & 0.00131                                    & 0.00226                                    \\ 
                        &GPT4Rec-LLaMA & 0.00000 & 0.00000 & 0.00000 & 0.00018 & 0.00027 & 0.00000 & 0.00000 & 0.00000 & 0.00054 & 0.00089 \\     
                        & DROS &0.00024&	0.00048&	0.00056&	0.00080&	0.00105&	0.00024&	0.00065&	0.00083&	0.00161&	0.00262 \\
                        & P5 & 0.00042&	0.00077&	0.00089&	0.00110&	0.00140&	0.00042&	0.00107&	0.00137&	0.00202&	0.00321\\
                        \cline{2-12} 
                        & \cellcolor[HTML]{EFEFEF}\textbf{BIGRec (1024)} & \cellcolor[HTML]{EFEFEF}\textbf{0.00488}   & \cellcolor[HTML]{EFEFEF}\textbf{0.00893}   & \cellcolor[HTML]{EFEFEF}\textbf{0.01069}   & \cellcolor[HTML]{EFEFEF}\textbf{0.0129}    & \cellcolor[HTML]{EFEFEF}\textbf{0.01589}   & \cellcolor[HTML]{EFEFEF}\textbf{0.00488}   & \cellcolor[HTML]{EFEFEF}\textbf{0.01189}   & \cellcolor[HTML]{EFEFEF}\textbf{0.01624}   & \cellcolor[HTML]{EFEFEF}\textbf{0.02307}   & \cellcolor[HTML]{EFEFEF}\textbf{0.03503}   \\
\multirow{-7}{*}{Games} & \cellcolor[HTML]{D0D0D0}\textbf{Improve}     & \cellcolor[HTML]{D0D0D0}\textbf{4000.05\%} & \cellcolor[HTML]{D0D0D0}\textbf{2392.93\%} & \cellcolor[HTML]{D0D0D0}\textbf{2366.02\%} & \cellcolor[HTML]{D0D0D0}\textbf{1852.36\%} & \cellcolor[HTML]{D0D0D0}\textbf{1513.20\%} & \cellcolor[HTML]{D0D0D0}\textbf{4000.05\%} & \cellcolor[HTML]{D0D0D0}\textbf{2122.21\%} & \cellcolor[HTML]{D0D0D0}\textbf{2175.00\%} & \cellcolor[HTML]{D0D0D0}\textbf{1516.66\%} & \cellcolor[HTML]{D0D0D0}\textbf{1180.44\%} \\ \hline
\end{tabular}}
\end{table*}

==> Figure_Table/tab2_underline_backup.tex <==
\begin{table*}[]
\caption{
% The presented table showcases the performance outcomes obtained by testing on the balance test set subsequent to training with 1024 randomly chosen sequences from the training set. The entries that are bolded denote the most superior results, whereas the term "Improve" signifies the relative enhancement of the proposed method in comparison to the optimal results achieved by conventional models.
Performance of compared method on the balanced testing set under the few-show training setting (1024 samples). 


after Training with 1024 Random Sequences from Training Set. Bold Entries Indicate Best Results, 'Improve' Signifies Relative Enhancement of Proposed Method over Conventional Models.

}
\label{tab:unpop_1024}
\resizebox{0.98\textwidth}{!}{
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}
\begin{tabular}{cccccccccccc}
\hline
                        & Model                                        & NG@1                                        & NG@3                                        & NG@5                                       & NG@10                                      & NG@20                                      & HR@1                                        & HR@3                                        & HR@5                                       & HR@10                                      & HR@20                                                \\ \hline
                        & GRU4Rec                                      & 0.00010                                    & 0.00021                                    & 0.00029                                    & 0.00046                                    & 0.00071                                    & 0.00010                                    & \underline{0.00030}                                    & 0.00050                                    & \underline{0.00102}                                    & \underline{0.00205}                                    \\
                        & Caser                                        & 0.00010                                    & 0.00021                                    & 0.00029                                    & 0.00046                                    & \underline{0.00071}                                    & 0.00010                                    & \underline{0.00030}                                    & 0.00050                                    & \underline{0.00102}                                    & 0.00202                                    \\
                        & SASRec                                       & \underline{0.00013}                                    & \underline{0.00022}                                    & \underline{0.00030}                                     & \underline{0.00046}                                    & 0.00071                                    & \underline{0.00013}                                    & 0.00030                                    & \underline{0.00050}                                    & 0.00099                                    & 0.00198                                    \\ 
                        & GPT4Rec-LLaMA & 0.00010 & 0.00021 & 0.00029 & 0.00045 & 0.00070 & 0.00010 & 0.00030 & 0.00050 & 0.00099 & 0.00198 \\
                        & Flan-T5 & 0.00010 & 0.00021 & 0.00029 & 0.00045 & 0.00070 & 0.00010 & 0.00030 & 0.00050 & 0.00099 & 0.00198 \\
                        \cline{2-12} 
                        & \cellcolor[HTML]{EFEFEF}\textbf{GoalRec (Ours)} & \cellcolor[HTML]{EFEFEF}\textbf{0.00595}   & \cellcolor[HTML]{EFEFEF}\textbf{0.00694}   & \cellcolor[HTML]{EFEFEF}\textbf{0.00753}   & \cellcolor[HTML]{EFEFEF}\textbf{0.00836}   & \cellcolor[HTML]{EFEFEF}\textbf{0.00921}   & \cellcolor[HTML]{EFEFEF}\textbf{0.00595}   & \cellcolor[HTML]{EFEFEF}\textbf{0.00767}   & \cellcolor[HTML]{EFEFEF}\textbf{0.00909}   & \cellcolor[HTML]{EFEFEF}\textbf{0.01167}   & \cellcolor[HTML]{EFEFEF}\textbf{0.01514}   \\
\multirow{-5}{*}{Movie} & \cellcolor[HTML]{D0D0D0}\textbf{Improve}     & \cellcolor[HTML]{D0D0D0}\textbf{4399.98\%} & \cellcolor[HTML]{D0D0D0}\textbf{3006.47\%} & \cellcolor[HTML]{D0D0D0}\textbf{2373.99\%} & \cellcolor[HTML]{D0D0D0}\textbf{1711.41\%} & \cellcolor[HTML]{D0D0D0}\textbf{1190.85\%} & \cellcolor[HTML]{D0D0D0}\textbf{4399.98\%} & \cellcolor[HTML]{D0D0D0}\textbf{2477.78\%} & \cellcolor[HTML]{D0D0D0}\textbf{1733.32\%} & \cellcolor[HTML]{D0D0D0}\textbf{1038.71\%} & \cellcolor[HTML]{D0D0D0}\textbf{638.71\%}  \\ \hline
                        & GRU4Rec                                      & \underline{0.00012}                                    & 0.00034                                    & \underline{0.00043}                                    & 0.00064                                    & 0.00092                                    & \underline{0.00012}                                    & 0.00048                                    & \underline{0.00071}                                    & 0.00137                                    & 0.00250                                    \\
                        & Caser                                        & \underline{0.00012}                                    & \underline{0.00036}                                    & 0.00043                                    & \underline{0.00066}                                    & \underline{0.00098}                                    & \underline{0.00012}                                    & \underline{0.00054}                                    & \underline{0.00071}                                    & \underline{0.00143}                                    & \underline{0.00274}                                    \\
                        & SASRec                                       & \underline{0.00012}                                    & 0.00026                                    & 0.00041                                    & 0.00060                                     & 0.00084                                    & \underline{0.00012}                                    & 0.00036                                    & \underline{0.00071}                                    & 0.00131                                    & 0.00226                                    \\ 
                        &GPT4Rec-LLaMA & 0.00000 & 0.00000 & 0.00000 & 0.00018 & 0.00027 & 0.00000 & 0.00000 & 0.00000 & 0.00054 & 0.00089 \\                  
                        &Flan-T5 & 0.00000 & 0.00000 & 0.00000 & 0.00011 & 0.00020 & 0.00000 & 0.00000 & 0.00000 & 0.00036 & 0.00071 \\ 
                        \cline{2-12} 
                        & \cellcolor[HTML]{EFEFEF}\textbf{GoalRec (Ours)} & \cellcolor[HTML]{EFEFEF}\textbf{0.00488}   & \cellcolor[HTML]{EFEFEF}\textbf{0.00893}   & \cellcolor[HTML]{EFEFEF}\textbf{0.01069}   & \cellcolor[HTML]{EFEFEF}\textbf{0.0129}    & \cellcolor[HTML]{EFEFEF}\textbf{0.01589}   & \cellcolor[HTML]{EFEFEF}\textbf{0.00488}   & \cellcolor[HTML]{EFEFEF}\textbf{0.01189}   & \cellcolor[HTML]{EFEFEF}\textbf{0.01624}   & \cellcolor[HTML]{EFEFEF}\textbf{0.02307}   & \cellcolor[HTML]{EFEFEF}\textbf{0.03503}   \\
\multirow{-5}{*}{Games} & \cellcolor[HTML]{D0D0D0}\textbf{Improve}     & \cellcolor[HTML]{D0D0D0}\textbf{4000.05\%} & \cellcolor[HTML]{D0D0D0}\textbf{2392.93\%} & \cellcolor[HTML]{D0D0D0}\textbf{2366.02\%} & \cellcolor[HTML]{D0D0D0}\textbf{1852.36\%} & \cellcolor[HTML]{D0D0D0}\textbf{1513.20\%} & \cellcolor[HTML]{D0D0D0}\textbf{4000.05\%} & \cellcolor[HTML]{D0D0D0}\textbf{2122.21\%} & \cellcolor[HTML]{D0D0D0}\textbf{2175.00\%} & \cellcolor[HTML]{D0D0D0}\textbf{1516.66\%} & \cellcolor[HTML]{D0D0D0}\textbf{1180.44\%} \\ \hline
\end{tabular}}
\end{table*}

==> Figure_Table/tab3_backup.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
% \usepackage[normalem]{ulem}
% \useunder{{ine}{{}{}
\begin{table*}[]
\caption{
Performance comparison of full-data training baselines and BIGRec trained with only 1024 samples on normal testing sets. `Pop' refers to the popularity-based item recommendation. The best results are highlighted in Bold.  The second largest value is marked with an underscore.}
\label{tab:full_training_result}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
% \usepackage[normalem]{ulem}
% \useunder{{ine}{{}{}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
% \usepackage[normalem]{ulem}
% \useunder{{ine}{{}{}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
% \usepackage[normalem]{ulem}
% \useunder{{ine}{{}{}
\begin{tabular}{cccccccccccc}
\hline
\rowcolor[HTML]{FFFFFF} 
                        & Model                                        & NG@1                                        & NG@3                                        & NG@5                                       & NG@10                                      & NG@20                                      & HR@1                                        & HR@3                                        & HR@5                                       & HR@10                                      & HR@20                                      \\ \hline
\multicolumn{12}{c}{Single model} \\
\cdashline{2-12} 
% \rowcolor[HTML]{FFFFFF} 
\cellcolor[HTML]{FFFFFF}                        & Pop                  & 0.0032                           & 0.0076                           & 0.0088                           & 0.0121                            & 0.0170                            & 0.0032                           & 0.0108                           & 0.0138                           & 0.0244                            & 0.0438                            \\
\rowcolor[HTML]{FFFFFF} 
\cellcolor[HTML]{FFFFFF}                        & GRU4Rec              & 0.0047                 & 0.0108                           & 0.0151                           & 0.0237                            & 0.0351                            & {{0.0047}}                     & 0.0155                           & 0.0259                           & 0.0527                            & 0.0985                            \\
\rowcolor[HTML]{FFFFFF} 
\cellcolor[HTML]{FFFFFF}                        & Caser                & 0.0045                           & 0.0113                           & 0.0161                           & 0.0242                            & {{0.0354}}             & 0.0045                           & 0.0165                           & 0.0281                           & {{0.0537}}                      & {{0.0986}}             \\
\rowcolor[HTML]{FFFFFF} 
\cellcolor[HTML]{FFFFFF}                        & SASRec               & 0.0045                           & {{0.0119}}                     & {{0.0171}}                     & 0.0268                   & 0.0389                   & 0.0045                           & {{0.0175}}                     & 0.0302                  & 0.0606                   & 0.1088                   \\
\rowcolor[HTML]{FFFFFF} & DROS & 0.0087	& 0.0186	& 0.0245	& 0.0359	& 0.0493	& 0.0087	& 0.0261	& 0.0406	& 0.0761	& 0.1292 \\
\rowcolor[HTML]{EFEFEF}
\cellcolor[HTML]{FFFFFF}                        & \textbf{BIGRec (1024)} & \textbf{0.0182 }                 & 0.0219                  & 0.0235                  & {{0.0262}}             & 0.0287                            &\textbf{ 0.0182}                  & 0.0247                  & {{0.0284}}            & 0.0369                            & 0.0471                            \\ 

\cline{2-12} 
% \rowcolor[HTML]{D0D0D0} 
% \multirow{-6}{*}{\cellcolor[HTML]{FFFFFF}Movie} & \textbf{Improve}     & \textbf{284.51\%}                & \textbf{84.18\%}                 & \textbf{37.71\%}                 & \textbf{-2.08\%}                  & \textbf{-26.18\%}                 & \textbf{284.51\%}                & \textbf{40.87\%}                 & \textbf{-5.96\%}                 & \textbf{-39.11\%}                 & \textbf{-56.71\%}                 \\
\multicolumn{12}{c}{SASRec enhanced model} \\
\cdashline{2-12} 
& Caser & 0.0046& 0.0119 & 	0.0167 & 	0.0272 & 	0.0409 &	0.0046& 	0.0173& 	0.0301&	0.0615 &	0.1159\\
\rowcolor[HTML]{EFEFEF}
\cellcolor[HTML]{FFFFFF} 
& \textbf{BIGRec (1024)} & \textbf{0.0182}	& \underline{0.0233} & 	\underline{0.0281} & 	\underline{0.0375} & 	0.0491 & 	\textbf{0.0182} & 	\underline{0.0272} & 	0.0388	& 0.0693 &	0.1151\\
\cline{2-12} 
\multicolumn{12}{c}{DROS enhanced model} \\
\cdashline{2-12} 
& Caser & 0.0087 & 0.0183 & 	0.0247 & 	0.0354 &	\underline{0.0494} & 	0.0087 & 	0.0258 & 	0.0404 & 	\underline{0.0756} & 	\underline{0.1296} \\
& SASRec & \underline{0.0089} & 	0.0184 & 	0.0245 & 	0.0357 & 	0.0493 & 	\underline{0.0089} & 	0.0256 & 	\underline{0.0409} & 	0.0754 & 	\textbf{0.1307} \\
\rowcolor[HTML]{EFEFEF}
\cellcolor[HTML]{FFFFFF} 
\multirow{-14}{*}{\cellcolor[HTML]{FFFFFF}Movie} & \textbf{BIGRec (1024)} & \textbf{0.0182}& \textbf{0.0256} &	\textbf{0.0325} & 	\textbf{0.0419} &	\textbf{0.0537} & 	\textbf{0.0182}&	\textbf{0.0317} & 	\textbf{0.0481} & 	\textbf{0.0776}&	0.1239 \\
\hline
\multicolumn{12}{c}{\textbf{Single model}} \\
\cdashline{2-12} 
% \rowcolor[HTML]{FFFFFF} 
\cellcolor[HTML]{FFFFFF}                        & Pop                  & 0.0000                           & 0.0000                           & 0.0000                           & 0.0004                            & 0.0018                            & 0.0000                           & 0.0000                           & 0.0000                           & 0.0014                            & 0.0068                            \\
\rowcolor[HTML]{FFFFFF} 
\cellcolor[HTML]{FFFFFF}                        & GRU4Rec              & 0.0051                           & 0.0080                           & 0.0094                           & 0.0109                            & 0.0129                            & 0.0051                           & 0.0101                           & 0.0135                           & 0.0184                            & 0.0263                            \\
\rowcolor[HTML]{FFFFFF} 
\cellcolor[HTML]{FFFFFF}                        & Caser                & 0.0059                           & 0.0094                           & 0.0111                           & 0.0141                            & 0.0177                            & 0.0059                           & 0.0119                           & 0.0161                           & 0.0256                            & {{0.0401}}                      \\
\rowcolor[HTML]{FFFFFF} 
\cellcolor[HTML]{FFFFFF}                        & SASRec               & {{0.0113}}                     & {{0.0151}}                     & {{0.0164}}                     & {{0.0185}}                      & {{0.0204}}                      & {{0.0113}}                     & {{0.0179}}                     & {{0.0209}}                     & {{0.0275}}                      & 0.0353                            \\ 
\cellcolor[HTML]{FFFFFF}                        & P5-small             & 0.0094	& 0.0124	& 0.0132	& 0.0151	& 0.0175	& 0.0094	& 0.0146	& 0.0164	& 0.0224	& 0.0320\\
\cellcolor[HTML]{FFFFFF}                        & P5-base              & 0.0094	& 0.0116	& 0.0131	& 0.0145 & 	0.0167	& 0.0094	& 0.0134 & 0.0172	& 0.0216	& 0.0300 \\
\cellcolor[HTML]{FFFFFF}                        & DROS &  0.0156	& 0.0194	& 0.0213	& 0.0244	& 0.0278	& 0.0156	& 0.0221	& 0.0269	& 0.0365	& 0.0500 \\
\cline{2-12}
\rowcolor[HTML]{EFEFEF} 
\cellcolor[HTML]{FFFFFF}                        & \textbf{BIGRec (1024)} & 0.0141                  & 0.0180                  & 0.0202                  & 0.0225                   & 0.0259                   & 0.0141                  & 0.0209                 & 0.0261                 & 0.0333                   & 0.0468                   \\
\rowcolor[HTML]{EFEFEF}
\cellcolor[HTML]{FFFFFF}           
& \textbf{BIGRec (full)} & \textbf{0.0219 }&	0.0245 &	0.0269	& 0.0295 &	
0.0319 &	0.0219	& 0.0264 &	0.0324 &	0.0403 &	0.0497  \\
\cline{2-12}
\multicolumn{12}{c}{\textbf{SASRec enhanced model}} \\
\cdashline{2-12} 
& Caser & 0.0131 &	0.0163 &	0.0182 &	0.0208 &	0.0243 &	0.0131 &	0.0189 &	0.0240 &	0.0317 &	0.0465\\
\rowcolor[HTML]{EFEFEF}
\cellcolor[HTML]{FFFFFF} 
& \textbf{BIGRec (1024)} & 0.0141 & 0.0228 &	0.0243 &	0.0265 &	0.0288 &	0.0141 &	0.0284 &	0.0326 & 0.0394 &	0.0507 \\
\rowcolor[HTML]{EFEFEF}
\cellcolor[HTML]{FFFFFF} 
& \textbf{BIGRec (full)} &  \textbf{0.0219}	& \underline{0.0268}	& \underline{0.0279}& 0.0299& 0.0330& \textbf{0.0219}& 0.0301& 0.0331&	0.0412&	0.0517 \\
\cline{2-12} 
\multicolumn{12}{c}{\textbf{DROS enhanced model}} \\
\cdashline{2-12} 
& Caser &\underline{0.0159}	& 0.0199 &	0.0217 &	0.0249 &	0.0288 &	\underline{0.0159} &	0.0227 &	0.0279 &	0.0375 &	0.0529\\
& SASRec & 0.0151 &	0.0197 &	0.0216 &	0.0247 &	0.0279 &	0.0151 &	0.0226 & 	0.0279 &	0.0373 &	0.0488\\
\rowcolor[HTML]{EFEFEF}
\cellcolor[HTML]{FFFFFF} 
 & \textbf{BIGRec (1024)} & 0.0141 &	0.0251	 & 0.0273 &	\underline{0.0308}	& \underline{0.0345}	& 0.0141& 	\underline{0.0325}&	\underline{0.0375} & \textbf{0.0484} &	\textbf{0.0630} \\
\rowcolor[HTML]{EFEFEF}
\cellcolor[HTML]{FFFFFF} 
\multirow{-18}{*}{\cellcolor[HTML]{FFFFFF}Game} & \textbf{BIGRec (full)} &\textbf{0.0219} &	\textbf{0.0291} &\textbf{0.0311} & \textbf{0.0337} &	\textbf{0.0372} &	\textbf{0.0219} &	\textbf{0.0341} &	\textbf{0.0387} &	\underline{0.0475} &	\underline{0.0615} 
% \rowcolor[HTML]{CECDCD} 
% \multirow{-6}{*}{\cellcolor[HTML]{FFFFFF}Games} & \textbf{Improve}     & \textbf{25.44\%}                 & \textbf{19.55\%}                 & \textbf{23.48\%}                 & \textbf{21.77\%}                  & \textbf{26.51\%}                  & \textbf{25.44\%}                 & \textbf{16.79\%}                 & \textbf{24.84\%}                 & \textbf{21.12\%}                  & \textbf{16.81\%}         
\\ \hline
\end{tabular}
\end{table*}

==> Figure_Table/tab3_underline_backup.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
% \usepackage[normalem]{ulem}
% \useunder\underline{{ine}\underline{{}{}
\begin{table*}[]
\caption{This table displays the results of baselines obtained from training on the full sample, followed by testing on the normal test. Distinguished from the baseline, our approach still employed only 1024 samples for training. ``Pop'' refers to the practice of recommending items based on their popularity within the training dataset. The bold indicates the best model performance, while the underlined represents the second-best outcome.}
\label{tab:full_training_result}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
% \usepackage[normalem]{ulem}
% \useunder{\underline{ine}{\underline{}{}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
% \usepackage[normalem]{ulem}
% \useunder{\underline{ine}{\underline{}{}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
% \usepackage[normalem]{ulem}
% \useunder{\underline{ine}{\underline{}{}
\begin{tabular}{cccccccccccc}
\hline
\rowcolor[HTML]{FFFFFF} 
                        & Model                                        & N@1                                        & N@3                                        & N@5                                       & N@10                                      & N@20                                      & R@1                                        & R@3                                        & R@5                                       & R@10                                      & R@20                                      \\ \hline
\rowcolor[HTML]{FFFFFF} 
\cellcolor[HTML]{FFFFFF}                        & Pop                  & 0.0032                           & 0.0076                           & 0.0088                           & 0.0121                            & 0.0170                            & 0.0032                           & 0.0108                           & 0.0138                           & 0.0244                            & 0.0438                            \\
\rowcolor[HTML]{FFFFFF} 
\cellcolor[HTML]{FFFFFF}                        & GRU4Rec              & {\underline{ 0.0047}    }                 & 0.0108                           & 0.0151                           & 0.0237                            & 0.0351                            & {\underline{ 0.0047}}                     & 0.0155                           & 0.0259                           & 0.0527                            & 0.0985                            \\
\rowcolor[HTML]{FFFFFF} 
\cellcolor[HTML]{FFFFFF}                        & Caser                & 0.0045                           & 0.0113                           & 0.0161                           & 0.0242                            & {\underline{ 0.0354}}             & 0.0045                           & 0.0165                           & 0.0281                           & {\underline{ 0.0537}}                      & {\underline{ 0.0986}}             \\
\rowcolor[HTML]{FFFFFF} 
\cellcolor[HTML]{FFFFFF}                        & SASRec               & 0.0045                           & {\underline{ 0.0119}}                     & {\underline{ 0.0171}}                     & \textbf{0.0268}                   & \textbf{0.0389}                   & 0.0045                           & {\underline{ 0.0175}}                     & {\textbf{ 0.0302} }                    & \textbf{0.0606}                   & \textbf{0.1088}                   \\
\rowcolor[HTML]{EFEFEF} 
\cellcolor[HTML]{FFFFFF}                        & \textbf{GoalRec (Ours)} & \textbf{0.0182}                  & \textbf{0.0219}                  & \textbf{0.0235}                  & {\underline{ 0.0262}}             & 0.0287                            & \textbf{0.0182}                  & \textbf{0.0247}                  & {\underline{ 0.0284}}            & 0.0369                            & 0.0471                            \\ \cline{2-12} 
\rowcolor[HTML]{D0D0D0} 
\multirow{-6}{*}{\cellcolor[HTML]{FFFFFF}Movie} & \textbf{Improve}     & \textbf{284.51\%}                & \textbf{84.18\%}                 & \textbf{37.71\%}                 & \textbf{-2.08\%}                  & \textbf{-26.18\%}                 & \textbf{284.51\%}                & \textbf{40.87\%}                 & \textbf{-5.96\%}                 & \textbf{-39.11\%}                 & \textbf{-56.71\%}                 \\
\rowcolor[HTML]{FFFFFF} 
\hline
\cellcolor[HTML]{FFFFFF}                        & Pop                  & 0.0000                           & 0.0000                           & 0.0000                           & 0.0004                            & 0.0018                            & 0.0000                           & 0.0000                           & 0.0000                           & 0.0014                            & 0.0068                            \\
\rowcolor[HTML]{FFFFFF} 
\cellcolor[HTML]{FFFFFF}                        & GRU4Rec              & 0.0051                           & 0.0080                           & 0.0094                           & 0.0109                            & 0.0129                            & 0.0051                           & 0.0101                           & 0.0135                           & 0.0184                            & 0.0263                            \\
\rowcolor[HTML]{FFFFFF} 
\cellcolor[HTML]{FFFFFF}                        & Caser                & 0.0059                           & 0.0094                           & 0.0111                           & 0.0141                            & 0.0177                            & 0.0059                           & 0.0119                           & 0.0161                           & 0.0256                            & {\underline{ 0.0401}}                      \\
\rowcolor[HTML]{FFFFFF} 
\cellcolor[HTML]{FFFFFF}                        & SASRec               & {\underline{ 0.0113}}                     & {\underline{ 0.0151}}                     & {\underline{ 0.0164}}                     & {\underline{ 0.0185}}                      & {\underline{ 0.0204}}                      & {\underline{ 0.0113}}                     & {\underline{ 0.0179}}                     & {\underline{ 0.0209}}                     & {\underline{ 0.0275}}                      & 0.0353                            \\ \cline{2-12} 
\rowcolor[HTML]{EFEFEF} 
\cellcolor[HTML]{FFFFFF}                        & \textbf{GoalRec (Ours)} & \textbf{0.0141}                  & \textbf{0.0180}                  & \textbf{0.0202}                  & \textbf{0.0225}                   & \textbf{0.0259}                   & \textbf{0.0141}                  & \textbf{0.0209}                  & \textbf{0.0261}                  & \textbf{0.0333}                   & \textbf{0.0468}                   \\
\rowcolor[HTML]{CECDCD} 
\multirow{-6}{*}{\cellcolor[HTML]{FFFFFF}Games} & \textbf{Improve}     & \textbf{25.44\%}                 & \textbf{19.55\%}                 & \textbf{23.48\%}                 & \textbf{21.77\%}                  & \textbf{26.51\%}                  & \textbf{25.44\%}                 & \textbf{16.79\%}                 & \textbf{24.84\%}                 & \textbf{21.12\%}                  & \textbf{16.81\%}         
\\ \hline
\\ \hline
\end{tabular}
\end{table*}

==> Figure_Table/tab_dataset_static.tex <==
% \begin{table}[t]
% \small
% \caption{Statistics of datasets.}
% \label{tab:dataStatics}
% \renewcommand\arraystretch{1.1}
% \begin{tabular}{cccc}
% \hline
% Dataset&MovieLens 10M&Video Games \\ \hline
% \#sequences& 9,301,274 & 149,796 \\
% \#items&10,682 &17,408 \\
% \#interactions& 10,000,054 & 496,315\\ \hline

% \end{tabular}
% \vspace{-1em}
% \end{table}

==> Figure_Table/table_4.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}
\begin{table*}[]
\begin{tabular}{ccccccccccc}
\hline
Model                                       & NG@1                                        & NG@3                                        & NG@5                                       & NG@10                                      & NG@20                                      & HR@1                                        & HR@3                                        & HR@5                                       & HR@10                                      & HR@20                                      \\ 
GRU4Rec                                                & \cellcolor[HTML]{FFFFFF}0.0051                               & \cellcolor[HTML]{FFFFFF}0.0080                              & \cellcolor[HTML]{FFFFFF}0.0094                              & \cellcolor[HTML]{FFFFFF}0.0109                              & \cellcolor[HTML]{FFFFFF}0.0129                              & \cellcolor[HTML]{FFFFFF}0.0051                               & \cellcolor[HTML]{FFFFFF}0.0101                              & \cellcolor[HTML]{FFFFFF}0.0135                              & \cellcolor[HTML]{FFFFFF}0.0184                              & \cellcolor[HTML]{FFFFFF}0.0263                      \\
Caser                                                 & \cellcolor[HTML]{FFFFFF}0.0059                               & \cellcolor[HTML]{FFFFFF}0.0094                              & \cellcolor[HTML]{FFFFFF}0.0111                              & \cellcolor[HTML]{FFFFFF}0.0141                              & \cellcolor[HTML]{FFFFFF}0.0177                              & \cellcolor[HTML]{FFFFFF}0.0059                               & \cellcolor[HTML]{FFFFFF}0.0119                              & \cellcolor[HTML]{FFFFFF}0.0161                              & \cellcolor[HTML]{FFFFFF}0.0256                              & \cellcolor[HTML]{FFFFFF}0.0401                      \\ 
            P5     & \cellcolor[HTML]{FFFFFF}0.0094                               & \cellcolor[HTML]{FFFFFF}0.0116                              & \cellcolor[HTML]{FFFFFF}0.0131                              & \cellcolor[HTML]{FFFFFF}0.0145                              & \cellcolor[HTML]{FFFFFF}0.0167                              & \cellcolor[HTML]{FFFFFF}0.0094                               & \cellcolor[HTML]{FFFFFF}0.0134                              & \cellcolor[HTML]{FFFFFF}0.0172                              & \cellcolor[HTML]{FFFFFF}0.0216                              & \cellcolor[HTML]{FFFFFF}0.0300                      \\ 
SASRec                                                 & \cellcolor[HTML]{FFFFFF}0.0113                               & \cellcolor[HTML]{FFFFFF}0.0151                              & \cellcolor[HTML]{FFFFFF}0.0164                              & \cellcolor[HTML]{FFFFFF}0.0185                              & \cellcolor[HTML]{FFFFFF}0.0204                              & \cellcolor[HTML]{FFFFFF}0.0113                               & \cellcolor[HTML]{FFFFFF}0.0179                              & \cellcolor[HTML]{FFFFFF}0.0209                              & \cellcolor[HTML]{FFFFFF}0.0275                              & \cellcolor[HTML]{FFFFFF}0.0353                      \\ \hline
DROS                                                 & \cellcolor[HTML]{FFFFFF}0.0156                               & \cellcolor[HTML]{FFFFFF}0.0194                              & \cellcolor[HTML]{FFFFFF}0.0213                              & \cellcolor[HTML]{FFFFFF}0.0244                              & \cellcolor[HTML]{FFFFFF}0.0278                              & \cellcolor[HTML]{FFFFFF}0.0156                               & \cellcolor[HTML]{FFFFFF}0.0221                              & \cellcolor[HTML]{FFFFFF}0.0269                              & \cellcolor[HTML]{FFFFFF}0.0365                              & \cellcolor[HTML]{FFFFFF}\textbf{0.0500}             \\ 
                                 \cellcolor[HTML]{EFEFEF}\textbf{BIGRec (1024)}             & \cellcolor[HTML]{EFEFEF}0.0141                               & \cellcolor[HTML]{EFEFEF}0.0180                              & \cellcolor[HTML]{EFEFEF}0.0202                              & \cellcolor[HTML]{EFEFEF}0.0225                              & \cellcolor[HTML]{EFEFEF}0.0259                              & \cellcolor[HTML]{EFEFEF}0.0141                               & \cellcolor[HTML]{EFEFEF}0.0209                              & \cellcolor[HTML]{EFEFEF}0.0261                              & \cellcolor[HTML]{EFEFEF}0.0333                              & \cellcolor[HTML]{EFEFEF}0.0468                      \\
                                 \cellcolor[HTML]{D0D0D0}\textbf{Improve }         & \cellcolor[HTML]{D0D0D0}-9.40\%                              & \cellcolor[HTML]{D0D0D0}-6.96\%                             & \cellcolor[HTML]{D0D0D0}-5.29\%                             & \cellcolor[HTML]{D0D0D0}-7.88\%                             & \cellcolor[HTML]{D0D0D0}-7.03\%                             & \cellcolor[HTML]{D0D0D0}-9.40\%                              & \cellcolor[HTML]{D0D0D0}-5.72\%                             & \cellcolor[HTML]{D0D0D0}-2.73\%                             & \cellcolor[HTML]{D0D0D0}-8.78\%                             & \cellcolor[HTML]{D0D0D0}-6.40\%                     \\ 
      \hline
\end{tabular}
\end{table*}


==> backup/experiments_0809.tex <==

\section{Experiments}
\label{section:exp}
In this section, we conduct experiments to answer the following research questions: 
\begin{itemize}[leftmargin=*]
\item RQ1: 
How does the performance of our BIGRec model compare to existing methods, when trained on a limited sample of 1024 data points?
\item RQ2: 
How is the performance of our model while simultaneously grounding the LLM to different actual items spaces?
\item RQ3: 
How does the performance of our model trained with limited data compare to that of traditional 
 recommendation models trained with  100 or even 1,000 times more samples in the same domain?
\item RQ4:
Can the LLM-based recommendation model achieve significant performance improvement with increasing data similar to traditional models? 
\item RQ5: 
To what extent does incorporating popularity information and collaborative features during model grounding improve its performance?

\end{itemize}



\input{Figure&Table/pop_count}

\subsection{Experimental Settings}
\subsubsection{Datasets.} We conduct experiments on two datasets:
\begin{itemize}[leftmargin=*]
    \item \textbf{Movie.} This refers to the well-known benchmark dataset for movie recommendation --- MovieLens10M\footnote{https://grouplens.org/datasets/movielens/10m/}.
    
    \item \textbf{Game.} This is a video-games recommendation dataset from Amazon\footnote{https://jmcauley.ucsd.edu/data/amazon/} and we use its 5-core subset. 
\end{itemize}


We chose the two datasets intentionally, as they exhibit different characteristics with regard to popularity bias. 
The Movie dataset reveals a significant bias toward popular items, while the Game dataset demonstrates a lesser degree of bias. 
Figure~\ref{fig:pop_count} illustrates the frequency of interactions across items with different levels of popularity, confirming that the Game dataset presents a more equitable distribution of interactions between popular and unpopular items than the Movie dataset. 
This suggests a lower degree of popularity bias in the Game dataset. Additional statistics for both datasets are summarized in Table~\ref{tab:dataStatics}.

 


To simulate real-world sequential recommendation scenarios, we divided each dataset into 10 periods based on the timestamp of the interactions. Subsequently, we split the periods of each dataset into training, validation, and testing sets\footnote{Due to limitations in the inference speed of LLM models, we randomly sample 5,000 validation and testing interactions as the final validation and testing sets, respectively.} using a ratio of 8:1:1. This approach ensures that the predicted interactions during testing come after all interactions observed during training, preventing the leakage of the testing phase information~\cite{ji2023critical} during training model. This is more akin to real-world situations~\cite{refCTR,ji2023critical}.


% In order to better simulate sequential recommendation scenarios in the real world, for each dataset, we first sort the sequences according to their timestamps, and then divide them into train, validation, and test sets based on the ratio of 8:1:1, in accordance with their chronological order. 
% \zjz{This ensures that the predicted interactions during testing occur later in time than the interactions observed during training, which is more aligned with real-world scenarios.}
% Table.\ref{tab:dataStatics} shows the static information of two datasets.

\subsubsection{Evaluation Protocols.}
% 遵循先前的工作，我们通过在测试阶段向模型输入一个序列，然后让模型预测用户会交互的下一个物品是什么来度量模型的性能。
Following the previous work~\cite{DRO1, SASRec}, we take the input historical interaction sequence for each testing interaction as the set of interactions that happened immediately prior to it. 
This approach allows for the possibility of including interactions that occur during the testing phase in the input sequence. 
To evaluate the model's performance, we use two commonly used evaluation metrics: Hit Ratio (HR) and Normalized Discounted Cumulative Gain (NDCG), which we compute using the all-ranking protocol. 
In this protocol, all items that a user has not interacted with are considered potential candidates.

\subsubsection{Compared Method}
To demonstrate the superiority of our method in the sequential recommendation, we compare it against the following conventional sequential recommendation methods and state-of-the-art LLM-based sequential recommendation methods:


\begin{itemize}[leftmargin=*]
    \item[-] \textbf{GRU4Rec~\cite{GRU4Rec}.} This is an RNN-based model that uses Gated Recurrent Units (GRU) to encode the user's past interactions with items and generate recommendations based on the learned patterns.
    
    \item[-] \textbf{Caser~\cite{Caser}.} It is a CNN-based model that represents the sequence of recent items as an image and uses convolutional filters in both horizontal and vertical directions to capture sequential patterns.
    In our implementation, we use one vertical filter and 16 horizontal filters with searching the height in \{2, 3, 4\}.

    \item[-] \textbf{SASRec~\cite{SASRec}.} This is a self-attention-based model that uses a causal (left-to-right) attention mechanism to learn sequential patterns and predict the next item. 
    
    \item[-] \textbf{P5~\cite{P5}} This approach leverages a combination of item IDs and natural language templates to undergo training for various recommendation tasks\footnote{
    For a fair comparison, we exclusively retain the task of sequence recommendation and its corresponding multiple templates during the training process.
    }.

    \item[-] \textbf{DROS~\cite{DRO1}} This is the state-of-the-art sequential recommendation method that employs distributionally robust optimization techniques to enhance its robustness against distributional changes.
    
    \item[-] \textbf{GPT4Rec-LLaMA~\cite{GPT4Rec}} is a modified version of the language model-based recommendation approach, GPT4Rec. The original method uses GPT-2 to generate hypothetical "search queries" based on a user's historical data, which are then searched using the BM25 search engine\footnote{We use the Rank-BM25 package at \url{https://github.com/dorianbrown/rank_bm25}.} to retrieve recommended items 
    % \bkq{which can be considered as another way to implement our second step of grounding}
    .
    To ensure a fair comparison, we have replaced the GPT-2 model with the LLaMA-7B model and performed model tuning using the LORA technique.    
    

\end{itemize}

We primarily utilize decoder-only LLMs as the backbone LLM model in our \textbf{BIGRec} method, given their prominent roles in the LLMs field. 
Specifically, we have chosen LLaMA-7B as our default choice for this study. 
% However, to investigate the impact of LLM model architecture, we also implement an alternative version called \textbf{BIGRec-T5}, which uses an encoder-decoder type of LLM model - Flan-T5-11B, currently the top-performing model in the T5 series~\cite{T5}. 
In addition to GPT4Rec, there are other existing LLM-based recommendation methods, such as TALLRec~\cite{bao2023tallrec}. 
However, since these methods are not applicable to our all-ranking setting, we do not compare them in our study.

\input{Figure&Table/tab_dataset_static}


\input{Figure&Table/tab1}

\input{Figure&Table/RQ4_figure}


\subsubsection{Implementation Details}
% 
We implement all of our methods using PyTorch. 
To preprocess the data, we first pad user interaction history with lengths less than 11 to a fixed length of 11. Then, we use a sliding window of length 11 to extract sequences, where the last item in each sequence is used as the prediction target and the preceding items form the input sequence. 
For all conventional models, we optimize them using the binary cross-entropy loss and uniformly sample negative samples. We use the Adam~\cite{Adam} as the optimizer with a tuned learning rate of $1e-3$, a batch size of 1024, and tune the weight decay in the range of $[1e\text{-}2, 1e\text{-}3, 1e\text{-}4, 1e\text{-}5, 1e\text{-}6, 1e\text{-}7]$. 
Regarding the hyperparameters of the conventional model architectures, we set their embedding size to 64 and the dropout ratio to 0.1. 
As suggested by the original papers, we only use one GRU layer for GRU4Rec; 
for SASRec, we set the number of self-attention heads and blocks to 1. 
We implemented DROS based on SASRec, as it performs the best in most scenarios among the three conventional sequential recommendation methods. 
For LLM-based methods, we follow the Alpaca setting~\cite{alpaca}, directly set the learning rate to $1e-4$, and use the AdamW~\cite{AdamW} optimizer.
For the hyperparameters of BM25, we follow the tuning range provided in GPT4Rec~\cite{GPT4Rec} paper. 
    For all methods, we use the early stop strategy with the patience of 20 epochs to select the best model and report the average results for three random seeds.
% 在利用公式X引入流行度信息和协同信息的过程中，我们发现由于scale的不一样，
For the hyperparameters of $\gamma$ in Eq.~(\ref{eq:eq2}), due to the disparate calculation methods employed by traditional models and LLM-based recommendation models, when incorporating information, we conducted a detailed search for a balanced integration of both approaches\footnote{Range from 0 to 1 with an increment of 0.01, and from 1 to 100 with an increment of 1.}.
% \todo{}



\subsection{Performance Comparison with Limited Training Data (RQ1)}
\label{sec:RQ1}
We first follow existing work~\cite{bao2023tallrec} to study the effectiveness of our method with limited training data (1024 training points).  
We compare it with the baselines trained with equivalent training samples. 
The comparison results results are summarized in Table~~\ref{tab:pop_1024}, where we draw the following main observations:
\begin{itemize}[leftmargin=*]
    \item When training data is limited, the conventional sequential baselines (GRU4Rec, Caser, SASRec) exhibit significantly worse performance than BIGRec implemented with LLM. These results are not surprising as these baselines rely on ID embeddings to build a recommender model, which is difficult to learn well with limited data. In contrast, BIGRec rapidly leverages the semantic knowledge of LLM obtained during the pre-training phase to achieve effective recommendations. These findings demonstrate the superiority of BIGRec over traditional recommendation models when dealing with limited training data. Furthermore, the improvement of BIGRec over these baselines in the top-ranked positions is much higher, indicating that BIGRec may tend to rank items of interest to users in higher positions. 

    \item While GPT4Rec-LLaMA is also LLM-based, it exhibits poor performance compared to BIGRec. We attribute this to the fact that BM25, which is used to ground the LLM outputs into actual items, is not suitable for the task. BM25 is a retrieval tool designed for document-level text. However, for the two datasets used in our study, the queries in GPT4Rec (item titles)  are very short. As a result, BM25 is susceptible to the impact of low-frequency word noise, making it difficult to accurately retrieve relevant items.

    % \item  
    % Despite using a larger Flan-T5-11B model and having relevant domain knowledge about the two datasets, BIGRec-T5, the encoder-decoder version of BIGRec, unexpectedly underperforms conventional recommender models. This may be attributed to inherent limitations of the encoder-decoder architecture, such as its relatively poor ability for generative tasks, as well as the potential need for more data to effectively learn a good sequence representation through the encoder.

    \item  The improvement of BIGRec over conventional models is significantly higher for the Game dataset compared to the Movie dataset. This difference is possibly due to the varying properties of popularity bias between the two datasets. Conventional methods tend to capture popular bias, while BIGRec is less affected by popularity bias. Therefore, conventional methods may perform better on the Movie dataset, in which \bkq{popular items play more dominant roles as evidenced by Figure~\ref{fig:pop_count}.}
    
\end{itemize}
·
%%% unpop 1024 setting
% \input{Figure&Table/tab2}

\input{Figure&Table/tab3}


\input{Figure&Table/Scaling_law}





% \par \textit{Performance on Balanced Testing.} 
% To further validate that our method is less susceptible to the popularity bias of the training dataset, we performed an additional experiment using a balanced testing setting. We followed the approach described in MACR~\cite{MACR} to adjust the testing distribution of items to be uniform and evaluated the model's performance. A model that is less affected by the popularity bias in the training data is expected to perform better in this balanced setting. We have summarized the results of all compared methods in Table~\ref{tab:unpop_1024}.

% As shown in the table, all models experience a noticeable decrease in performance compared to their results on the normal test setting presented in Table~\ref{tab:pop_1024}. 
% This can be attributed to the models' lack of knowledge about tail items or their inability to utilize the knowledge stored in LLMs for recommendation. 
% However, in this balanced testing setting, the performance improvement of BIGRec over conventional baselines is even greater than that observed in the normal test setting in Table~\ref{tab:pop_1024}. 
% This suggests that BIGRec may be superior for tail items, indicating that it is inherently less sensitive to the popularity bias of training data when compared to conventional recommendation models.

\subsection{Performance of Grounding to Multiple Actual Items Space (RQ2)}
 In addition to their ability to quickly learn new tasks, LLMs have the potential to serve as a universal processor for different actual items spaces.
 However, it is unclear whether this capability is retained after applying our grounding paradigm, \ie whether our grounding paradigm can ground LLMs to different actual items spaces simultaneously. 
 To explore this, we randomly selected 1024 samples from two domains (Movies and Game) to train our model and tested it on the testing sets of two domains, respectively.
 We compared the performance of this model with the model trained on single-domain data. 
 The results, depicted in Figure \ref{fig:multi_domain_result}, demonstrate that BIGRec trained on two-domain data performs comparably on each individual domain as compared to when it is trained on a single domain. 
 These findings suggest that BIGRec can simultaneously ground LLMs to different actual item spaces, at least at the level of different domains.




\subsection{Performance Comparison to Baselines Trained with More Data(RQ3)}
\label{sec:RQ3}
Given the impressive performance gains of BIGRec over baselines when trained on limited data, we are curious to investigate the extent of the gap that remains between BIGRec trained on limited data and the baselines trained with 100 or even 1,000 times more data.
Table~\ref{tab:full_training_result} presents the results of the baselines trained with more data, which consisted of over 7 million sequences for Movies and 120 thousand for Game, alongside the results of BIGRec trained with only 1024 samples\footnote{Due to the constraints of computational resources, we only present the results of baselines that consume significant computational resources on the Game dataset.}. 
From the table, we find that, compared to conventional baselines on the Movie data, BIGRec exhibits better performance at the top position of the recommendation list, but performs worse with regard to the relative bottom positions of the recommendation list. 
% Contrasting with the movie dataset findings, our method exhibits consistently superior performance to traditional models on the Video Games data except showing comparable with DROS which is a method that has been meticulously optimized within the traditional framework.
Contrary to the results obtained from the movie dataset, our method consistently demonstrates superior performance compared to traditional models when applied to the Game data. 
However, it should be noted that our method's performance is comparable to that of DROS, a meticulously optimized method within the traditional framework.
We draw two conclusions based on these results:
\begin{itemize}[leftmargin=*]
    \item Our method, BIGRec, trained on just 1,024 samples, could demonstrate comparable performance to conventional models trained with 100 or even 1,000 times more data in most cases, particularly when recommendation resources are limited. This highlights the practical applicability of LLMs for recommendations. Meanwhile, the results indicate that there is significant potential to enhance BIGRec's grounding by enlarging its training set and expanding its seen actual items during grounding, which may lead to further performance improvements.
    
    \item When compared to the Game dataset, the Movie dataset is denser and more heavily influenced by popularity bias (as evidenced by the performance of the Most-Pop methods on the two datasets). The difference in the performance gain of BIGRec between the two datasets suggests that BIGRec performs exceptionally well in scenarios where data is scarce and works effectively with less reliance on popularity bias. 
    \todo{Moreover, BIGRec (full) also}
    
\end{itemize}



\subsection{Performance of Different Training Samples (RQ4)}
\label{sec:RQ5}
% 基于前文的分析，我们看到在数据量增长的过程中，传统模型学到了大量的知识 (过去常常被称为协同信息)，受益于这些信息，传统模型能够大幅度提升他们的推荐能力，一个自然的想法是是否大模型也能通过增加数据量来学到这部分知识
Based on our previous analysis, it was observed that as the volume of data increased, traditional models acquired a substantial amount of knowledge, which was previously known as collaborative information.
This knowledge proved to be beneficial as it led to a significant enhancement in the recommendation abilities of these traditional models. 
To explore whether LLMs can also acquire this knowledge by increasing the amount of data, we conduct an analysis of the correlation between the volume of recommendation data and the performance of recommendations on the game dataset\footnote{The movie dataset comprises over 7M samples, making it challenging for us to train it comprehensively with LLM.}.
% 实验现象是
As shown in Figure~\ref{fig:scaling_law}, in comparison to traditional recommendation models, the incremental increase in data volume has a limited impact on the enhancement of LLM-based recommendations.
% Though for traditional models, game datasets are considered more challenging due to their sparsity. 
We believe this phenomenon is due to the strong semantic priors of LLMs, which tend to utilize their own semantic information to complete tasks while ignoring other valuable statistical information, such as popularity and collaborative information.


\input{Figure&Table/col_plot}


\input{Figure&Table/RQ3_figure}


% \subsection{Popularity Effectiveness for BIGRec (RQ2)}
\subsection{Performance on Introducing Popularity Information and Collaborative Features(RQ5)}

Given the heavy reliance on semantic information in LLMs, we believe the inclusion of suitable statistical information enhances the recommendation ability.
%%% TODO 加一个衔接解释一下为啥引入pop
Based on our observation in Section~\S\ref{sec:RQ1} and ~\S\ref{sec:RQ3}, we first study whether using the method presented in Eq.(\ref{eq:eq2}) to incorporate popularity information into the grounding of BIGRec could enhance its recommendation accuracy for Movie data, where popular items are particularly important.  
We compared the original version of BIGRec with the version that incorporates popularity information in Figure~\ref{fig:pop_enhanced}. 
The figure demonstrates that after incorporating popularity information, BIGRec achieves performance improvements for the NDCG@K and Recall@K metrics, particularly for larger values of $K$. 
Additionally, the performance is substantially better than when using only popularity information for recommendation (as shown in Table~\ref{tab:full_training_result}). 
These results indicate that injecting popularity information can be beneficial for grounding the output of LLMs to actual items in BIGRec, further enhancing its performance.

Furthermore, given the potential absence of collaborative information in LLMs, we integrate conventional models (\eg SASRec and DROS) as collaborative information into the LLM-based recommendation model. 
We then compare this approach with injecting information between two conventional recommendation models, as shown in Figure~\ref{fig:improve}
We draw two observations as follows:
\begin{itemize}[leftmargin=*]
    \item In the analysis of the movie dataset, the findings demonstrate that incorporating collaborative information into an LLM yields a more significant enhancement compared to incorporating information into a different conventional model. This confirms our initial assumption that LLM-based recommendation models lack that information.
    \item Incorporating SASRec as collaborative information on the game dataset resulted in the LLM-based recommendation model exhibiting comparable performance improvements to traditional models. However, when utilizing DROS as collaborative information, the model demonstrated clear advantages for improvements. We attribute this to the intrinsic difficulty of the game dataset and the insufficient learning exhibited by SASRec compared to DROS.
\end{itemize}
% \todo{figure or table and deeply analyze}
The above experiments indicate that there is significant potential for advancing recommendation accuracy even further by investigating more effective and efficient techniques for enhancing the grounding to the actual items space in BIGRec.


% The previous analysis highlighted the insensitivity of BIGRec towards popularity bias, but in certain scenarios, such as popularity-driven movie datasets, popularity can be quite important. 
% Is it possible to incorporate popularity information into the recommendations generated by LLMs? Our analysis in the grounding to the real-world stage indicates that simply utilizing a method similar to PDA~\cite{PDA} can enable large models to leverage popularity to enhance the performance of recommendations~\footnote{\zjz{
% We performed tuning $\gamma$ for each K based on the validation set performance using the parameter range specified in PDA~\cite{PDA}.}}. 
% % 考虑到这个实验分析的是在流行度重要的情景中的结果，我们在流行度主导的movie数据集上进行了测试。
% Given that this experiment examines the outcomes in a context where popularity is paramount, we conducted our testing on the movie dataset which is dominated by popularity.
% % 因为我们探究的是融入流行度增强模型性能的可行性，我们对每个K按照PDA~\cite{PDA}中的调参范围进行了调节。我们的实验证明了可以在grounding to the real-world阶段加入传统推荐中重要的统计信息比如流行度来增强模型的推荐性能，为未来进一步的探索提供了想象空间。

% % \todo{Detail setting for pop BIGRec}

% Based on the result, we have the following observations:
% \begin{itemize}
%     % 加入流行度之后，在K比较大的时候有明显的提升。这也符合之前的分析，大模型自然擅长K很小的推荐，加入流行度后有助于提高top 20这种相对比较大的K的推荐性能。
%     \item After incorporating popularity, there was a noticeable increase in performance when K was relatively large. This aligns with our previous analysis that LLMs are naturally better at recommending for smaller values of K, and adding popularity helps to improve the recommendation performance for larger values of K such as the top 20.
%     % 加入流行度之后，尾部的性能同时比直接使用BIGRec进行推荐和使用流行度推荐都高，这说明grounding to the real world 阶段的模型可以从流行度中受益，同时结合BIGRec和流行度的有点。
%     \item After incorporating popularity, the performance of the model on the tail end is higher compared to using either BIGRec or popularity-based recommendations alone. This indicates that the grounding to the real-world stage of the model can benefit from popularity, as well as the combination of BIGRec and popularity.
% \end{itemize}




% \input{Figure&Table/table_4}



% Given the explosive performance of the LLMs on the equivalent number of samples, a natural idea is to compare them to traditional models trained with far more data to gauge how much of a gap still remains for large models trained on small amounts of data.
% % 表3展示了大模型在1024个样本上训练的结果对比传统模型在所有sequence上训练的结果(8M for MovieLens10M, 110K for Video Games) PS: 这里只有训练集，没有用验证集和测试，比所有seq总数少
% Table 3 illustrates the performance of the LLMs, which are fitted employing a mere 1,024 samples, in apposition with the outcomes attained by traditional models that are trained on the entirety of the available sequences (amounting to over 7 million sequences for MovieLens10M and 120 thousand for Video Games)

% % 在电影数据集上，我们发现与传统模型相比，基于LLM的模型在头部仍然有巨大的性能提升，这表明了利用大模型的生成能力进行推荐的可行性
% On the movie dataset, we find that, in comparison to the traditional models, the LLM-based models fitted by our methodology continue to exhibit superior performance in the top ranks (over 200\% improvement on NDCG@1), indicating the feasibility of harnessing the generative capabilities of LLMs for recommendations.
% % 除此以外，我们发现传统模型相比于大模型的优势在于相对靠后的排序位置，这表明了基于大模型的生成式推荐仍然有很大潜力可以挖掘。
% In addition, we find that traditional models exhibited an advantage over LLMs with regard to the relative position of lower-ranked recommendations, indicating that there remains great untapped potential in generative recommendations based on LLMs.
% % 与电影数据集不同，在Video Games数据集上，我们的模型与传统模型在各个rank上有着一致的提升
% Contrasting with the findings for the movie dataset, on the Video Games data our methods exhibit uniformly superior performance to traditional models.

% 综合上面两个数据集来看，我们有以下总结
% Upon reviewing the findings across the two datasets, the following conclusions may be drawn:
% % 从整体上来看，我们的模型在1024样本上训练后的表现与传统模型在两个数据集上全量数据训练后的的表现相近，
% \begin{itemize}
%     \item 1) Our methods with training on a mere 1,024 samples show comparable performance \zjz{in most cases} with that of traditional models trained on the entirety of the two datasets, demonstrating the practical applicability of LLMs for recommendations, suggesting 
% % 在电影数据集上传统模型在相对考后的排序位置的表现, 除了数据抽密度和数据量的关系以外，还有可能源自于流行度对这个数据集的影响，如表中所示仅仅通过流行度的推荐方法(Most-Pop)明显更实用与MovienLens10M
%     \item 2)The superior performance of traditional models at the relative position of lower ranks in the MovieLens10M (@10 and @20), in addition to being attributable to data density and volume factors, may also stem from the effect of popularity on this particular data set. As shown in the table~\ref{tab:full_training_result}, a naive recommendation method based solely on popularity (Most-Pop) proves notably effective for MovieLens10M.
% \end{itemize}
% \todo{Ground vs Alignment
% Gournd abstract --> Concrete
% Alignment abstract --> abstract}


==> discussion.tex <==
% 1. time 曲线 
% \item beam search --> 提升性能， 带来的是time * gpu cost f
%       随着想要推荐的物品数增多  几乎线性增长


% \item currently LLM  (ChatGPT Claude LLaMA-chat) neural sampling 
%       diversity
% 最大化推荐性能



% If we use LLM 4 Rec we should balance this
%




% \item  1. 多次推荐 （exp）
% 2. 单次infer 多样性 没法评价

% future work 提一嘴

% 我们尝试了通过增大beam size让模型生成更多的推荐结果来推荐 , time consuming and gpu cost, 我们结合currently 的一些工作选择
% 增大beam search来获得更好的推荐结果是promising的



==> experiments_backup_0715.tex <==
\section{Experiments}
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}


% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}
 In this section, we conduct experiments to answer the following research questions: 
\begin{itemize}[leftmargin=*]

\item 
How does the performance of our model compare to existing methods, when trained on a limited sample of 1024 data points, in two different testing scenarios: one where popular items dominate and another with a balanced distribution of items?

 % \item RQ2: By introducing popularity information in a causal manner, can our model better ground to the real world where popularity bias exists?


    \item RQ3: By introducing popularity information in a causal manner, whether it is able to further boost our model's performance on a dataset dominated by popularity?
    \item RQ4: How is the performance of our model when conjunction training upon multi-domain data?
    \item RQ5: Does utilizing our model relative to traditionally trained models with complete data yield divergences, and where do the disparities lie if any?

    % \item RQ1: On equivalent samples (1024) and a test set dominated by popularity, does our model has advantages over traditional models?
    % \item RQ2: On equivalent samples (1024) and a test set balanced across all items, does our model has advantages over traditional models?

    % \item RQ3: By introducing popularity information in a causal manner, whether it is able to further boost our model's performance on a dataset dominated by popularity?
    % \item RQ4: How is the performance of our model when conjunction training upon multi-domain data?
    % \item RQ5: Does utilizing our model relative to traditionally trained models with complete data yield divergences, and where do the disparities lie if any?
\end{itemize}



\begin{figure}
    \centering
    \includegraphics[width=8cm]{Figure&Table/pop_count.pdf}
    \caption{This figure showcases the fluctuations in popularity of Movie and Games datasets. The abscissa indicates ten groups divided by popularity from high to low, while the logarithmic coordinate axis is employed to represent the proportion of interactions in this group to the total number of interactions.}
    \label{fig:pop_count}
\end{figure}

\subsection{Experiment Settings}
\subsubsection{Datasets.}
\begin{itemize}
    \item \textbf{Movie.} We use the real-world movie recommendation dataset MovieLens10M~\footnote{https://grouplens.org/datasets/movielens/10m/}. This dataset is one of the well-known datasets dominated by popularity.
    % In this dataset, we have filtered out users with an interaction history of less than 10.
    \item \textbf{Games.} This is a video-games recommendation dataset from Amazon~\footnote{https://jmcauley.ucsd.edu/data/amazon/}. Compared with MovieLens10M, this dataset is less influenced by popularity.
\end{itemize}
Figure.\ref{fig:pop_count} depicts the detailed popularity of two datasets. The horizontal axis divides the items into ten groups, based on their popularity, arranged from high to low. Meanwhile, the vertical axis is the logarithmic representation of the proportion of interactions within the group compared to the total number of interactions. It is evident that movies, aside from being ranked highest in the most popular group (group 0), are significantly below games in all other groups. This indicates that the bias in popularity for the movie dataset is much greater than that of games.

% 为了更好地模拟真实世界中的sequential 推荐场景，对于每个数据集我们首先按照时间序列对sequence进行排序，然后依据时间按照8：1：1进行划分train，valid和test.
In order to better simulate sequential recommendation scenarios in the real world, for each dataset, we first sort the sequences according to their timestamps, and then divide them into train, validation, and test sets based on the ratio of 8:1:1, in accordance with their chronological order. 
\zjz{This ensures that the predicted interactions during testing occur later in time than the interactions observed during training, which is more aligned with real-world scenarios.}
Table.\ref{tab:dataStatics} shows the static information of two datasets.

\subsubsection{Evaluation Protocols.}
% 遵循先前的工作，我们通过在测试阶段向模型输入一个序列，然后让模型预测用户会交互的下一个物品是什么来度量模型的性能。
Following previous work~\cite{SASRec}, we measure the performance of the recommendation model by inputting a sequence during the evaluation phase and letting the model predict the next item the user would interact with. 
% 为了高效地度量我们提出的方法在有流行度bias和无流行度bias下的性能，我们通过对验证集和测试集采样构造了有偏和无偏两种测试来度量我们模型的性能。
\todo{To efficiently evaluate the performance of our proposed method under popularity bias and no popularity bias, we constructed biased and unbiased settings by sampling from the validation and test sets.}


\input{Figure&Table/tab1}
\input{Figure&Table/tab2}

\begin{itemize}
    % 对于每个数据集，我们在划分好的验证集和测试集中随机采样了5000个用户历史交互和next item对来度量模型在有popularity bias下的性能表现。
    \item \textbf{Normal Test.} For each dataset, due to limitations in the inference speed of LLM models, we randomly sampled 5000 user histories and the next item pairs from the pre-defined validation and test sets to assess the model's performance under the normal item distribution
    % 对于验证集和测试集，我们为其中出现的每一个作为预测结果的item选取一条样本构成新的验证集和测试集
    \item \textbf{Balanced Test.} For each dataset, we select one user history and the next item pair for each item appears as a prediction result in the pre-defined validation and test sets to testify to the model's performance in an entirely balanced scenario.
    % For the validation set and test set, for each item that appears as a prediction result, we select one sample to constitute a new validation set and test set.
    % \item \todo{add a figure/table to show the popularity of the above two dataset} 
\end{itemize}

% 我们使用了两个被广泛使用的指标来度量模型的性能：hit ratio 和 normalized discounted cumulative gain
We utilized two widely-used metrics to measure the performance of the model: Hit Ratio (HR) and Normalized Discounted Cumulative Gain (NDCG).

\input{Figure&Table/tab_dataset_static}

\subsubsection{Baselines}
To showcase the superiority of our network structure in comparison to sequential temporal recommendation methods, we conducted a comparative analysis of three classical temporal recommendation algorithms.
\begin{itemize}
    \item \textbf{GRU4Rec~\cite{GRU4Rec}.} RNN-based sequential recommender, using GRU to encode the user's interaction history and do recommendations.
    \item \textbf{Caser~\cite{Caser}.} It is a CNN-based sequential recommender using horizontal and vertical convolution to capture the user's behaviors. One vertical filter and 16 horizontal filters with heights \{2, 3, 4\} are applied in our implementation. 
    \item \textbf{SASRec~\cite{SASRec}.} Self-attention-based sequential recommendation model, using attention mechanism to recommend the next item.
    \item \textbf{Flan-T5~\cite{T5}.} A recommender system based on an encoder-decoder architecture LLM, Flan-T5-11B, which is currently the best-performing model in the T5 series, is chosen for comparison as we directly applied our method to this model.
    \item \textbf{GPT4Rec-LLaMA~\cite{GPT4Rec}} This is utilizing a language model to generate a query and then conducting a search within the items using the BM25~\cite{BM25} search engine. We implement the BM25 with Rank-BM25 package~\footnote{\url{https://github.com/dorianbrown/rank_bm25}}. To ensure a fair comparison, we replaced the GPT2 model from the original paper with the LLaMA-7B model and performed lightweight finetuning using LoRA.
\end{itemize}

\subsubsection{Implementation Details}
% 
Our study utilizes Python 3.10 and PyTorch 2.0 to implement the proposed methods. 
In order to maintain consistent sequence lengths, we employ padding on sequences with a historical interaction length below a predetermined threshold of 10, utilizing `<pad>' tokens. 
% For historical interaction sequences with a length greater than 10, we have retained the last 10 interactions as the historical sequence.
\zjz{For user interaction history data with a length greater than 10, we utilized a sliding window of length 10 to construct the sequence that meets the length requirement.
The model needs to predict the user's next interaction item based on the provided sequence.}
For all traditional recommendation baselines, we use Adam~\cite{Adam} optimizer, the learning rate is tuned as $1e-3$ and the batch size is set as 1024. We tune the weight decay within the range of $[1e-2, 1e-3, 1e-4, 1e-5, 1e-6, 1e-7]$. We use the early stop with a patience of 20 epochs to select the best model. We use binary cross-entropy loss and uniform negative sampling to optimize the traditional recommendation baselines since this is an implicit feedback setting.
For LLM-based methods, we follow the alpaca setting~\cite{alpaca}, directly set the learning rate to $1e-4$, and use the AdamW~\cite{AdamW} optimizer. We report the average results for three random seeds.



\subsection{Performance Comparison on Equivalent Samples (RQ1, RQ2)}
% 首先为了验证我们的方法的有效性，我们首先在相同的样本上与传统方法对比
To ascertain the effectiveness of our proposed method, we initially compare it with traditional methods on equivalent samples (1024).
% 表1展示了baseline方法和我们的方法在常规数据集上的表现
Table~\ref{tab:pop_1024}  exhibit the performance of the baseline and our method on the normal test sets.
% 首先我们可以观察到，在有偏数据上基于ID的baseline差距不是很明显, 说明了这些传统的推荐模型在少数据量上没有本质的差别
Firstly, we observe that on the normal test set, the performance disparity of the ID-based baselines is not very pronounced, demonstrating that these conventional recommendation models lack intrinsic distinction in low-source settings.
% 对比我们基于Decoder大模型的方法，情理之中的是大模型利用其在预训练阶段学到的知识能够更快的通过语义进行推荐，相比于传统模型有着明显的优势，然而其在头部的明显提升仍然在我们的意料之外
Compared with our methodology leveraging a decoder-based LLM, it is reasonable that the LLM, by virtue of the knowledge obtained during the pre-training phase, may recommend more rapidly through semantics, manifesting a dominant over traditional recommendation models; yet, its salient improvement on the top-rank remains beyond our anticipation (Improved more than 600\% and 1000\% at NDCG@1 on the movie and video games dataset, respectively.

% 令我们惊讶的事情是, 同样的基于大模型的方法, Flan-T5-11B的模型却并没有展现出任何优势, 甚至比传统的推荐模型还要差, 尽管从参数量上他要大于LLaMA7B, 同时他也具有一定的领域知识(例如，询问Flan-T5-11B什么是钢铁侠，他能给出钢铁侠电影的相关知识）
What did surprise us is that the identical methodology leveraging Flan-T5-11B, failed to learn to recommend in a low-resource setting, in fact performing worse than traditional recommendation models, despite it being larger in parameters compared to LLaMA-7B and also possessing some domain knowledge (for instance, upon asking Flan-T5-11B what is Iron Man (II), it can furnish relevant information about the Iron Man (II) movie).
% 我们将这个现象归因于encoder-decoder架构对于生成式推荐任务在少样本上的天生劣势，一方面，encoder在对所有token做信息聚合的时候难免会丢失一部分信息，另一方面，通过encoder获得一个很好的用户表示可能需要更多的数据量来学习
We attribute this phenomenon to the innate disadvantage of the encoder-decoder architecture for generative recommendation tasks with fewer samples, on the one hand, the encoder inevitably loses some information when aggregating information for all tokens, and on the other hand, obtaining a good user representation through the encoder may require more data to learn from.
% 而另一个基于大模型的方法GPT4Rec-LLaMA, 同样表现出很差的推荐能力，我们认为这是因为BM25本身是一个适用于长文本检索的检索工具，而在电影和游戏领域，由于标题长度本身较短，因此BM25很容易受到低频词噪声的影响从而难以做到准确的召回
While another LLM-based method GPT4Rec-LLaMA also exhibits poor recommending capability which we attribute to the fact that BM25 is a retrieval tool apt for document-level text.
In domains like movie and video games, due to the inherent short length of titles, BM25 succumbs to the impact of low frequency word noise, making it difficult to accomplish accurate recall.
% 另一个有趣的发现是，我们的模型在Video_Games上相比于传统模型的性能提升要远高于在MovieLens10M上相比于传统模型的提升
Another interesting finding is that our model's performance enhancement over traditional models on Video Games is far more significant compared to the enhancement on MovieLens10M.
% 这个原因可能归结于多方面，一个重要的考量是流行度是否主导了该数据集的推荐结果. 
There may have been multiple contributing factors, a key consideration is that MovieLens10M  is a popularity-dominated dataset, so even with 1024 samples, traditional models can learn some popularity knowledge through the frequency of ID appearances.

% 为了进一步观察这个现象，我们在表2中展示了baseline模型和我们的模型在一个对于item来说均衡的数据集上的表现
To further observe this phenomenon, we demonstrate the performance of the baseline model and our methods on a balanced test set for items in Table~\ref{tab:unpop_1024}.
% 尽管我们观察到所有的模型相比于Normal的test set都有明显的下降, 这是由于在1024样本上很多样本是模型没有见过的，因此无论是大模型还是小模型都不知道可以把这类样本放进结果空间中考量
Although all models exhibited a noticeable drop compared with their performance on the normal test set, mainly because both the baseline models and LLMs are not seen many items before; therefore, they are not likely to know how to consider such items in their result spaces.
% 尤其是对大模型来说，即使他有这个item的信息，他仍然不知道怎么怎么把这个item考虑成一个结果
Notably for the LLMs, even when they had the requisite item knowledge, they still did not know how to consider that item as a solution for the recommendation problem at hand.
% 然鹅，我们仍然发现了大模型相比于传统模型的巨大提升，甚至比他在normal测试集上的提升还要明显
However, we are still nevertheless delighted to discover that the LLM shows a greater improvement over these traditional models, even higher than that improvement on the normal test set, over 4000\% improvement for both scenarios.
% 这表明了相比于传统模型，大模型在学习过程中确实不易收到pop的影响
This indicates that the LLMs are innately less sensitive to popularity information in the learning process when compared to the traditional recommendation models.



\subsection{Popularity Effectiveness for GRec (RQ3)}
% 前文分析到了大模型的推荐结果天然对于流行度不敏感，但是在某些场景下面流行度有比较重要比如流行度主导的movie数据集。那么是否有可能将流行度信息引入到大模型推荐中去呢？我们发现直接在grounding to the reality阶段通过简单使用类似于PDA~\cite{PDA} 的方式，就可以使得大模型能够利用流行度提高推荐性能。
The previous analysis highlighted the insensitivity of the recommendation results of LLMs towards popularity, but in certain scenarios, such as popularity-driven movie datasets, popularity can be quite important. Is it possible to incorporate popularity information into the recommendations generated by LLMs? Our analysis in the grounding to the real-world stage indicates that simply utilizing a method similar to PDA~\cite{PDA} can enable large models to leverage popularity to enhance the performance of recommendations. 
% 考虑到这个实验分析的是在流行度重要的情景中的结果，我们在流行度主导的movie数据集上进行了测试。
Given that this experiment examines the outcomes in a context where popularity is paramount, we conducted our testing on the movie dataset which is dominated by popularity.
% 因为我们探究的是融入流行度增强模型性能的可行性，我们对每个K按照PDA~\cite{PDA}中的调参范围进行了调节。我们的实验证明了可以在grounding to the real-world阶段加入传统推荐中重要的统计信息比如流行度来增强模型的推荐性能，为未来进一步的探索提供了想象空间。
\zjz{[Check: I am wondering whether or not the topic of hyperparameter tuning will be discussed here.]
As we were examining the feasibility of integrating the enhancement of model performance through increased popularity, we made adjustments to each K according to the tuning range specified in PDA~\cite{PDA}. Our experiments have demonstrated that incorporating crucial statistical information such as popularity into the grounding to the real-world phase of traditional recommendation can indeed enhance the model's recommendation performance, thereby providing room for further exploration in the future.}
\todo{Detail setting for pop GRec}

Based on the result, we have the following observations:
\begin{itemize}
    % 加入流行度之后，在K比较大的时候有明显的提升。这也符合之前的分析，大模型自然擅长K很小的推荐，加入流行度后有助于提高top 20这种相对比较大的K的推荐性能。
    \item After incorporating popularity, there was a noticeable increase in performance when K was relatively large. This aligns with our previous analysis that LLMs are naturally better at recommending for smaller values of K, and adding popularity helps to improve the recommendation performance for larger values of K such as the top 20.
    % 加入流行度之后，尾部的性能同时比直接使用GRec进行推荐和使用流行度推荐都高，这说明grounding to the real world 阶段的模型可以从流行度中受益，同时结合GRec和流行度的有点。
    \item After incorporating popularity, the performance of the model on the tail end is higher compared to using either GRec or popularity-based recommendations alone. This indicates that the grounding to the real-world stage of the model can benefit from popularity, as well as the combination of GRec and popularity.
\end{itemize}
The mere enhancement of the grounding to the real-world stage through a simple way has led to significant improvements in the performance of GRec. This leaves us with vast room for imagination. The exploration of more effective and efficient means to improve the grounding to the real-world stage is an intriguing open problem.


\begin{figure}
    \centering
    \begin{subfigure}
        \centering
        \includegraphics[width=4cm]{Figure&Table/RQ3_NDCG.pdf}
        % \includegraphics[width=4.5cm]{figure.pdf}
    \end{subfigure}
    \begin{subfigure}
        \centering
        \includegraphics[width=4cm]{Figure&Table/RQ3_HR.pdf}
    \end{subfigure}
    \caption{This figure displays the improvement in performance after incorporating popularity in the grounding to the real-world stage, as compared to before its inclusion. The left side showcases the NDCG results for varying Top k values, while the right side exhibits the HR results.}
    \label{fig:pop_enhanced}
\end{figure}

\subsection{Is Multi-Domain Decrease the Performance?(RQ4)}
% LLMs 除了能够快速学会一个新的任务以外，还具有极强的跨域泛化能力。为了验证在经过我们提出的grounding范式之后，LLM是否还保留类似的能力，我们构建了一个multi domain的测试场景。
LLMs exhibit robust cross-domain generalization abilities in addition to being able to quickly learn new tasks. To determine whether LLMs retain similar capabilities after undergoing our proposed grounding paradigm, we devised a multi-domain testing environment.
%具体而言，我们首先从movie和games两个数据集中随机选出1024个samples，合在一起构造instruction供大模型进行instruction tunning训练，然后我们分别在movie和games单独测试训练好的模型，查看它相对于只在单个数据集上训练，单个数据集上测试的结果的变化。
To be specific, we initially selected 1024 samples randomly from the movie and games datasets and combined them to form instructions for the large model to undergo instruction tuning training. Subsequently, we tested the trained models separately on the movie and games datasets to observe the changes in the results compared to those obtained from training and testing on a single dataset just as illustrated in Figure.\ref{fig:multi_domain_result}. 

% 我们从实验结果中最主要的观察是我们提出的GRec在使用两个domain进行训练之后，可以分别在两个domain上取得和单个domian上训练推荐相当的性能，这体现了我们提出的GRec的强大的跨域推荐性能。
The primary observation from our experimental results is that our proposed GRec model, after being trained on two domains, can achieve comparable performance on each individual domain as compared to when it is trained on a single domain. This highlights the robust cross-domain recommendation performance of GRec.
% 具体而言，Figure中每个柱子的左边是multi domain训练，单个domain测试的结果，右边则是直接在该domain上训练并测试的结果。我们展示了两个数据集中不同K的NDCG和HR的结果。可以看见在所有情况下，GRec并没有因为domain变多而导致推荐性能出现显著下降而是体现出和comparable的结果
To be precise, the left side of each bar in the Figure.\ref{fig:multi_domain_result} shows the results of multi-domain training and single-domain testing, while the right side shows the results of training and testing directly on that domain. We present the NDCG and HR results for different values of K in two different datasets. 
In all scenarios, it can be observed that GRec did not exhibit a significant decrease in recommendation performance due to the increase in domains, but rather demonstrated comparable results.


\begin{figure*}[htbp] %通栏
\begin{minipage}[t]{0.23\linewidth} %调节两个子图左右间距
\centering
\includegraphics[width=1.65in, height=1.4in]{Figure&Table/RQ4_NDCG_movie.pdf} %调节单个子图大小
\end{minipage}%
\begin{minipage}[t]{0.23\linewidth}
\centering
\includegraphics[width=1.65in, height=1.4in]{Figure&Table/RQ4_HR_movie.pdf}
\end{minipage}%
\begin{minipage}[t]{0.23\linewidth}
\centering
\includegraphics[width=1.65in, height=1.4in]{Figure&Table/RQ4_NDCG_games.pdf}
\end{minipage}
\begin{minipage}[t]{0.23\linewidth}
\centering
\includegraphics[width=1.65in, height=1.4in]{Figure&Table/RQ4_HR_games.pdf}
\end{minipage}%
\caption{These four figures demonstrate the multi-domain results of our proposed method on the Movie and Games datasets. 
% The two figures on the left represent the results on the movie dataset, while the two figures on the right represent the results on the games dataset. 
The left bars in each column indicate the results of training and testing on a single domain, while the right bars indicate the results obtained by training on both the movie and games datasets, and subsequently testing on each dataset individually.}
\label{fig:multi_domain_result}
\end{figure*}


\input{Figure&Table/tab3}
\subsection{Performance Comparison with Full-finetuning Baselines (RQ5)}
% 基于大模型在相同数量sample上的表现如此炸裂，一个自然的想法是与更多训练数据量相比的传统模型比较，在少量样本上训练的大模型还有多少差距
Given the explosive performance of the LLMs on the equivalent number of samples, a natural idea is to compare them to traditional models trained with far more data to gauge how much of a gap still remains for large models trained on small amounts of data.
% 表3展示了大模型在1024个样本上训练的结果对比传统模型在所有sequence上训练的结果(8M for MovieLens10M, 110K for Video Games) PS: 这里只有训练集，没有用验证集和测试，比所有seq总数少
Table 3 illustrates the performance of the LLMs, which are fitted employing a mere 1,024 samples, in apposition with the outcomes attained by traditional models that are trained on the entirety of the available sequences (amounting to over 7 million sequences for MovieLens10M and 120 thousand for Video Games)
% 在电影数据集上，我们发现与传统模型相比，基于LLM的模型在头部仍然有巨大的性能提升，这表明了利用大模型的生成能力进行推荐的可行性
On the movie dataset, we find that, in comparison to the traditional models, the LLM-based models fitted by our methodology continue to exhibit superior performance in the top ranks (over 200\% improvement on NDCG@1), indicating the feasibility of harnessing the generative capabilities of LLMs for recommendations.
% 除此以外，我们发现传统模型相比于大模型的优势在于相对考后的排序位置，这表明了基于大模型的生成式推荐仍然有很大潜力可以挖掘。
In addition, we find that traditional models exhibited an advantage over LLMs with regard to the relative position of lower-ranked recommendations, indicating that there remains great untapped potential in generative recommendations based on LLMs
% 与电影数据集不同，在Video Games数据集上，我们的模型与传统模型在各个rank上有着一致的提升
Contrasting with the findings for the movie dataset, on the Video Games data our methods exhibit uniformly superior performance to traditional models.
% 综合上面两个数据集来看，我们有以下总结
Upon reviewing the findings across the two datasets, the following conclusions may be drawn:
% 从整体上来看，我们的模型在1024样本上训练后的表现与传统模型在两个数据集上全量数据训练后的的表现相近，
1) our methods with training on a mere 1,024 samples show comparable performance with that of traditional models trained on the entirety of the two datasets, demonstrating the practical applicability of LLMs for recommendations, suggesting 
% 在电影数据集上传统模型在相对考后的排序位置的表现, 除了数据抽密度和数据量的关系以外，还有可能源自于流行度对这个数据集的影响，如表中所示仅仅通过流行度的推荐方法(Most-Pop)明显更实用与MovienLens10M
2)The superior performance of traditional models at the relative position of lower ranks in the MovieLens10M (@10 and @20), in addition to being attributable to data density and volume factors, may also stem from the effect of popularity on this particular data set. As shown in the table~\ref{tab:full_training_result}, a naive recommendation method based solely on popularity (Most-Pop) proves notably effective for MovieLens10M.

\todo{Ground vs Alignment
Gournd abstract --> Concrete
Alignment abstract --> abstract}

